Strong Byzantine Agreement with Adaptive Word Complexity

The strong Byzantine agreement (SBA) problem is defined among n processes, out of which t < n can be faulty and behave arbitrarily. SBA allows correct (non-faulty) processes to agree on a common value. Moreover, if all correct processes have proposed the same value, only that value can be agreed upon. It has been known for a long time that any solution to the SBA problem incurs quadratic worst-case word complexity; additionally, the bound was known to be tight. However, no existing protocol achieves adaptive word complexity, where the number of exchanged words depends on the actual number of faults, and not on the upper bound. Therefore, it is still unknown whether SBA with adaptive word complexity exists. This paper answers the question in the affirmative. Namely, we introduce STRONG, a synchronous protocol that solves SBA among n = (2 + Omega(1))t + 1 processes and achieves adaptive word complexity. We show that the fundamental challenge of adaptive SBA lies in efficiently solving certification, the problem of obtaining a constant-sized, locally-verifiable proof that a value can safely be decided.

==> old/certification_with_low_resiliency.tex <==
\section{Certification phase for $n = a\cdot t+1$ with $a\leq 4$}

First Round (SUBMIT):

Every process $i$ sends its value $v_i$ to the leader. with partial signature $PS^{t+1}_i(v_i)$ for threshold of $t+1$.  The leader receives a set $V$ of values with $|V| \in [n-t, t]$.  If the leader is correct and receives $t+1$ times the same value $v^{*}$,  then it can compute a threshold signature $TS^{t+1}(v^{*})$ for $v^{*}$ $TS^{t+1}_i(v^{*})$ which proves that at least one correct process proposed $v^{*}$ and so proves that deciding $v^{*}$ cannot violate validity.
Hence,  we consider the case (*) where it does not exist any value received $t+1$ times by the leader.
In that case, the leader can partition the received values $V$ into $(G_j)_{j \in J}$ as follows:
\begin{enumerate}
\item $|G_1| \leq ... \leq |G_{|J|}| $ by construction
\item $\forall j \in [2:|J|],  |G_j| \leq t$ (by (*)) \label{item:star}
\item $\forall (i,j) \in J^2,  |G_i| + |G_j| > t $  \label{item:pair-lower-than-t} (a pair that does not verify this predicate can always be merged into a new one that still verifies the previous property \ref{item:star}. Then this procedure can be repeated recursively until property  \ref{item:pair-lower-than-t}  is verified).
\item $|J| \in [a+1,  2 a]$.  The lower bound comes from property \ref{item:star}, the upper bound comes from property \ref{item:pair-lower-than-t}.
\end{enumerate}

Second Round (CONFIRM):

For every $j \in J$,  for every process $i$ that sent a value $v_i \in G_j$ The leader sends a predicate $P_j$ describing the set $G_j$ to process $i$.  If the predicate indeed corresponds to the value previously sent,  the process $i$ signs $P_j$ with $\tau$ different share signatures  with as many thresholds : $\frac{q \cdot t}{\tau}$ for $q \in [1:\tau]$.

Final Round (PROOF):

For each $j \in J$ the leader receives $z_j$ (well-formed) CONFIRM messages (from correct or non-correct processes).
Since $\forall j \in J,  \exists q_j \in [1:\tau]$ s.t.  $z_j \in [\frac{q_j \cdot t}{\tau}: \frac{(q_j + 1) \cdot t}{\tau} - 1]$,   $\forall j \in J$,
the leader can prove the predicate $P_j$ has been signed by $\frac{q_j \cdot t}{\tau}$ processes (via threshold signature $TS^{\frac{q_j \cdot t}{\tau}}(P_j)$) that is by at least $z_j - \frac{t}{\tau} + 1$.

%For each $j \in J$,  $|G_j| \geq x_j$ where $x_j$ is the number of correct processes that sent a value in $G_j$.  Thus,  for each $j \in J$ the leader receives at least $x_j$ CONFIRM messages.
%Since $\forall j \in J,  \exists q_j \in [1:\tau]$ s.t.  $x_j \in [\frac{q_j \cdot t}{\tau}: \frac{(q_j + 1) \cdot t}{\tau} - 1]$,   $\forall j \in J$,  the leader can prove the predicate $P_j$ has been signed by $\frac{q_j \cdot t}{\tau}$ processes (via threshold signature $TS^{\frac{q_j \cdot t}{\tau}}(P_j)$) that is by at least $x_j - \frac{t}{\tau} + 1$.

We note $S = \sum_{j \in J}( z_j - \frac{t}{\tau} + 1) > Z - \frac{2at}{\tau} $ with $Z = \sum_{j \in J}z_j $.

Since $Z \geq n-t$, we have $S > n-t  -  \frac{2at}{\tau}$

%For $a = 4$ and $\tau = 8$, we obtain  $S \geq n-2t \geq 2t+1$.

The leader can prove, with no more than $|J|$ threshold signatures, that $S$ different processes signed values in (at least 3) pairwise disjoints subsets where each subset is represented by at most $t$ processes.  Thus, if $S \geq 2t+1$,  the leader can prove at least two different values have been proposed by two different correct processes and so  any value can be decided without strong unanimity violation.
This is the case for $a=4$ and $\tau = 8$.

\section{Certification phase for $n = 3\cdot t+1$}

We apply the same structure.
The difference appears in the final round. 

Here again, the leader collects $S > Z - \frac{2at}{\tau}$ signatures that can be merged into no more than $|J|$ threshold signatures. Let us fix $\tau = 12$. Then $S > Z - \frac{t}{2}$.
If $Z \geq (2t+1) + \frac{t}{2}$, then $S \geq (2t+1)$ and we are done.

Otherwise $Z \leq (2t+1) + \frac{t}{2}$, which means the number of faulty processes $f \geq n-Z \geq \frac{t}{2}$, i.e. $f = O(n)$ ! In that case, the leader can  put all the $Z$ CONFIRM messages in a full-certificate (with $Z=O(n)$ words) and broadcast the full-certificate and we are done. 

\section{Certification phase for $n = (2+c)\cdot t+1$ with $c \in ]0:1]$}

We apply the same structure.
The difference appears in the final round. 

Here again, the leader collects $S > Z - \frac{2(2+c)t}{\tau}$ signatures, that can be merged into no more than $|J|$ threshold signatures.
Since $Z \geq n-f$, 
We can write $S > n-f - \frac{2(2+c)t}{\tau}$ and then $S > (2t+1) + (c - \frac{2(2+c)}{\tau})t - f$.

Let us fix $\tau = \frac{4(2+c)}{c}$. Then $S > (2t+1) + \frac{ct}{2} - f$.

We can apply the same reasoning.

If $f \leq \frac{ct}{2}$, $Z \geq (2t+1)$ and we are done.

Otherwise $f = O(n)$ ! In that case, the leader can  put all the $Z$ CONFIRM messages in a full-certificate (with $Z=O(n)$ words) and broadcast the full-certificate and we are done. 

Some big constants appears here. For $c = 0.5$, $\tau = 20$ and the big certificate is sent with $f = \frac{n}{10}+1$ only.
For $c = 0.1$, $\tau = 84$ and the big certificate is sent with $f = \frac{n}{42}+1$ only.

\fi

==> sections/approval.tex <==
\section{Optimistic Approval}

In this section, we define the Optimistic Approval task, that intuitively allows correct processes to agree on a common valid value under some optimistic conditions, while safety is never violated even under more pessimistic conditions.

The $(f_0,p_\ell)$-approval task is a distributed task among $n$ processes exposing the following interface: (1) request $\mathit{submit}(v)$ - a process submit a value $v$; invoked at most once, (2) indication $\mathit{approve}(v)$ - a process approves the value $v$, (3) indication $\mathit{abort}()$ - a process does not approve any value. The $(f_0,p_\ell)$-approval task ensures:
\begin{itemize}
    \item (Strong Validity) If all the correct processes submit a value $v$, then no value $v' \neq v$ can be approved.
    %\item (Agreement) No pairs of correct processes approve two different values.
    \item (Optimistic Approval) If (1) process $p_{\ell}$ (the leader) is correct and (2) the actual number of Byzantine processes is $f \leq f_0$, then all correct processes approve a common (valid) value.
    \item (Synchronization) If all the correct processes submit a value at the same round, then all the correct processes output an indication (approve or abort) at the same round.
\end{itemize}

In the authenticated model that we assume, this task is trivial to implement. Indeed, it is sufficient that each correct process sends its signed proposal to the leader, that wait for $n-f_0$ message, concatenate them and broadcast the batch, where the most represented value can be safely approved. 
However, the communication complexity of this naive solution would be quadratic.
The challenge is to implement this task with a linear communication complexity.



==> sections/certificate_collecting.tex <==
\section{\cert}

We present \cert, a certification protocol which plays the crucial role in \name.
\textsc{bucket} solves the certification problem in $O(1)$ synchronous rounds, while exchanging only $O(n)$ bits.
Without loss of generality, we assume that \cert performs certification of natural numbers ($\mathsf{Value} = \mathbb{N}$). % \pierre{Of course, $\mathbb{N}$ is in bijection with $\{0,1\}^{*}$.}.

First, we introduce positive and negative certificates (\Cref{subsection:positive_negative}).
Then, we describe \textsc{bucket}, and present its pseudocode.
Finally, we reason about the correctness and complexity of \textsc{bucket}. 

\subsection{Positive \& Negative Certificates} \label{subsection:positive_negative}

The leader drives the certification in \cert (as we explain in \Cref{subsection:cert_description}).
Intuitively, processes report their starting values to the leader.
Then, the leader's responsibility is, given the received starting values, to construct a certificate for some value.
Depending on the received starting values, the leader constructs either (1) a positive, or (2) a negative certificate.
% We explain these below.
% \textsc{bucket} distinguishes two types of certificates.

\paragraph{Positive certificates.}
A certificate is positive if it proves that ``enough'' processes have started \cert with the same value.
Specifically, if a certificate proves that $t + 1$ processes have started with the same value, then the certificate is \emph{positive}.
Observe that a value accompanied by a positive certificate is necessarily a starting value of one correct process.
% is always ``safe'' as the certificate shows that some correct process has started \textsc{bucket} with that value.

% In \textsc{bucket}, obtaining positive certificates is easy (as explained in \Cref{subsection:bucket_description}).
% Moreover, a positive certificate is a $(t + 1)$-combined signature.
% Attainment of a positive certificate in \textsc{bucket} is possible only if (at least) $t + 1$ correct processes start \textsc{bucket} with the same value.

\paragraph{Negative certificates.}
A certificate is said to be \emph{negative} if it proves that \emph{not all} correct processes have started \cert with the same value.
Concretely, a negative certificate (1) includes information about the starting values of (at least) $2t + 1$ processes, and (2) it proves that, amongst \emph{these} $2t + 1$ processes, no $t + 1$ processes have started \cert with the same value.
If a negative certificate is constructed, it is guaranteed that not all correct processes have started with the same value.
Indeed, if all correct process started with the same value, among any set of $2t + 1$ starting values, there would (at least) $t + 1$ matching values, which implies that a negative certificate could \emph{not} have been constructed.
The question, however, is how we can prove, using only $O(1)$ signatures, that correct processes have started \cert with different values.

\subsection{Negative Certificates: Detailed Analysis}

The main challenge in designing \cert is ensuring that negative certificates include only $O(1)$ signatures.
As previously mentioned, a negative certificate carries information about $2t + 1$ starting values, while proving that, among these $2t + 1$ starting values, there is no ``$(t + 1)$-common'' value.
In this subsection, we explain how \cert produces constant-sized negative certificates.
% In this subsection, we provide a detailed analysis of the negative certificates, and how \textsc{bucket} ensures their constant size.

\paragraph{Problem.}
Suppose that the leader receives starting values from $X \geq 2t + 1$ processes such that, among these $X$ processes, no $t + 1$ processes have started \cert with the same value.
In this case, the leader cannot form a positive certificate; its goal is to create a negative certificate.
% In this case, the goal of the leader is to construct a negative certificate.
% given the received $X$ starting values.
A naive way for the leader to achieve this is to construct a negative certificate as a set of the $X$ received (and properly signed) messages.
Indeed, such a certificate would prove that not all correct processes have started with the same value.
The problem with such an implementation of negative certificates is that they would include $O(t)$ signatures; recall our goal of having constant-sized certificates.

\paragraph{Intuition behind solution.}
When the leader receives the aforementioned $X \geq 2t + 1$ starting values, which do not allow the leader to form a positive certificate, the leader starts the \emph{partitioning}.
%First, the leader extracts $x$ (resp. $y$) to be the minimum (resp. maximum) value among the received starting values.
Namely, the leader partitions all of the received starting values into a set of $|G| = O(1)$ disjoint \emph{groups} such that each group contains starting values of at most $t$ processes. Each group $g_i$ of is associated with a description $g_i.\mathit{description}$ being an interval, such that $\bigcup_{i \in [1, |G|]} g_i.\mathit{description} = \mathbb{N}$ and $\bigcap_{i \in [1, |G|]} g_i.\mathit{description} = \emptyset$.
Then for each group $g$, the leader sends a request to the processes whose starting values do not belong to $g$ asking them to share-sign a statement ``My value does not belong to $g$''. 
Once the leader receives signatures for the group $g$, it combines them into a $(t+1)$-threshold signature proving that starting values of ``enough'' processes do not belong to $g$. 
If the leader is able to obtain a $(t+1)$-threshold signature per group (which is the case if $f \leq t_{\mathit{opt}} \triangleq c \cdot t$), the leader can construct a constant-sized negative certificate.
Indeed, for every value $v \in \mathbb{N}$, $v$ belong to a certain group $g$ in $G$ and so there is at least one correct process that did not propose value $v$.



%\paragraph{Intuition behind solution.}
%When the leader receives the aforementioned $X \geq 2t + 1$ starting values, which do not allow the leader to form a positive certificate, the leader starts the \emph{partitioning}. Namely, the leader partitions all of the received starting values into disjoint \emph{groups} such that each group contains starting values of at most $t$ processes. Then, for each constructed group $g$, the leader sends a request to the processes whose starting values belong to $g$ asking them to share-sign a statement ``My value belongs to $g$''. Once the leader receives signatures for the group $g$, it combines them into a threshold signature proving that starting values of ``enough'' processes belong to $g$. If the leader is able to obtain $O(1)$ threshold signatures which prove that (1) there exist at least $3$ disjoint groups, and (2) the starting values of (at least) $2t + 1$ processes belong to these three groups, the leader can construct a constant-sized negative certificate. Indeed, the starting values of (at least) $t + 1$ correct processes are included in the aforementioned $3$ groups. As no group contains the starting values of more than $t$ processes, the certificate proves that two correct processes have proposed different values.

\paragraph{Partitioning.}
Let us start by defining \emph{groups}; as previously mentioned, the leader partitions all received starting values into disjoint groups.
Each group $g$ has the following attributes:
\begin{compactitem}
    \item $g.\mathsf{description} = [x \in \mathsf{Value}, y \in \mathsf{Value}]$: This field represents a description of starting values which belong to the group $g$.
    Intuitively, if there exists a starting value $v$ such that $x \leq v \leq y$, then the leader includes $v$ in the group $g$.
    
    % Moreover, we define the \emph{precedence} relation between two group descriptions.
    Given two group description $\mathit{desc}_1 = [x_1, y_1]$ and $\mathit{desc}_2 = [x_2, y_2]$, $\mathit{desc}_2$ \emph{follows} $\mathit{desc}_1$ (we write ``$\mathit{desc}_1 \follows \mathit{desc}_2$'') if and only if $x_1 +1 \leq y_1 +1 = x_2 \leq y_2 $. 
    % For example, $g.\mathsf{description} = [1, 5]$ implies that all starting values
    % associates all starting values $x$ with (1) $1 \leq x \leq 5$, or (2) $7 \leq x \leq 10$ with the group $g$.
    For any value $v$ and any group description $\mathit{desc} = [x, y]$, we define the $\mathsf{match}(v, \mathit{desc}) \in \{\mathit{true}, \mathit{false}\}$ function:
    \begin{equation*}
        \mathsf{match}(v, \mathit{desc}) = \mathit{true} \iff x \leq v \leq y.
    \end{equation*}
    
    \item $g.\mathsf{processes}$: This field denotes the processes whose starting values are included in the group $g$ according to $g.\mathsf{description}$.
    Formally:
    \begin{equation*}
        g.\mathsf{processes} = \{ P_i \,|\, \mathsf{match}(P_i\text{'s starting value}, g.\mathsf{description}) = \mathit{true}\}.
    \end{equation*}
    Moreover, $|g.\mathsf{processes}| \leq t$: a group contains starting values of (at most) $t$ processes.
    For example, let $P_1$ start with $1$, $P_2$ start with $3$, and $P_3$ start with $7$.
    Let $g$ be a group such that $g.\mathsf{description} = [1, 4]$.
    Then, $g.\mathsf{processes} = \{P_1, P_2\}$.
\end{compactitem}

A \emph{group-partitioning} is an array $G$ of groups such that:
\begin{compactitem}
    \item (Compactness) $|G| = O(1)$
    \item (Partitioning) $min(G[1]) = 0$, $max(G[|G|]) = +\infty$, and $\forall i \in [1:|G|-1], G[i] \follows G[i+1]$
\end{compactitem}

How does the leader partition all received starting values?
To this end, we introduce the $\mathsf{partition}$ function.
We present a simplified pseudocode of the $\mathsf{partition}$ function below; we give a detailed pseudocode in \Cref{appendix:partition}.

\begin{algorithm} [ht]
% \caption{The $\mathsf{partition}$ function}
% \label{algorithm:partition}
% \caption*{My Algorithm}
\addcontentsline{loa}{algorithm}{My Algorithm}
\begin{algorithmic} [1]

\State \textbf{function} $\mathsf{partition}(\mathsf{Array}\big( (\mathsf{Process}, \mathsf{Value}) \big) \text{ } \mathit{process\_value\_array})$:
\State \hskip2em $\mathit{process\_value\_array}.\mathsf{sort\_by\_value}()$ \BlueComment{sort the array according to the starting values}
\State \hskip2em \textcolor{blue}{\(\triangleright\) form groups containing a single starting value}
\State \hskip2em $\mathsf{Array}(\mathsf{Group})$ $\mathit{groups} \gets \mathsf{form\_identical\_values\_groups}()$
\State \hskip2em $\mathit{groups}.\mathsf{sort\_by\_value}()$ \BlueComment{sort the array according to the starting values}
\State \hskip2em $\mathit{groups}.\mathsf{merge\_adjacent\_groups}()$ \BlueComment{merge adjacent groups when possible} \label{line:merge_partition}
\State \hskip2em $\mathit{groups}.\mathsf{expand\_descriptions}()$ \BlueComment{expand descriptions to ensure Partitioning property} \label{line:expand_description}
\State \hskip2em \textbf{return} $\mathit{groups}$
\end{algorithmic}
\end{algorithm}


The $\mathsf{partition}$ function returns an array of groups $\mathsf{G}$, which is sorted according to the descriptions of the groups.

%More formally, the following holds for $\mathsf{G}$:
%\begin{compactenum}
   % \item $\mathsf{G}$ is an array of groups such that, for every $i \in [1, |\mathsf{G}| - 1]$, $\mathsf{G}[i].\mathsf{description} \prec \mathsf{G}[i + 1].\mathsf{description}$.
  %  That is, $\mathsf{G}$ is an array sorted according to the descriptions of the groups.
    
   % \item For every $i \in [1, |\mathsf{G}| - 1]$, $|\mathsf{G}[i].\mathsf{processes} + \mathsf{G}[i + 1].\mathsf{processes}| \geq t + 1$.
   % That is, two adjacent groups have starting values of (at least) $t + 1$ processes; otherwise, they would be ``merged'' into the same group at line~\ref{line:merge_partition} of the $\mathsf{partition}$ function.
%\end{compactenum}

The crucial feature of the $\mathsf{partition}$ function is that it constructs $O(1)$ groups, which we prove below.

\begin{theorem}
Let $\mathsf{G}$ be an array of groups returned by the $\mathsf{partition}$ function.
Then, $|\mathsf{G}| = O(1)$.
\end{theorem}
\begin{proof}
For every $i \in [1, |\mathsf{G}| - 1]$, $|\mathsf{G}[i].\mathsf{processes} + \mathsf{G}[i + 1].\mathsf{processes}| \geq t + 1$.
    That is, two adjacent groups have starting values of (at least) $t + 1$ processes; otherwise, they would be ``merged'' into the same group at line~\ref{line:merge_partition} of the $\mathsf{partition}$ function.
Recall that $n = (2 + c)t + 1$, for some fixed constant $c \in (0,1]$.
Moreover, for every $i \in [1, |\mathsf{G}| - 1]$, $|\mathsf{G}[i] + \mathsf{G}[i + 1]| \geq t + 1$.
Hence:
\begin{equation*}
    |\mathsf{G}| \leq \lceil 2 \cdot \frac{n}{t + 1} \rceil \leq \lceil 2 \cdot \frac{(2 + c)t + 1}{t + 1} \rceil < \lceil 2 \cdot \frac{(2 + c)(t + 1) + (t + 1)}{t + 1} \rceil \leq \lceil 2 \cdot (3 + c) \rceil.
\end{equation*}
Thus, $|\mathsf{G}| < \lceil 2 \cdot (3 + c) \rceil$, which concludes the proof.
\end{proof}

%After obtaining $G$ from the partitioning function, the leader build an array $S = (s_1, ..., s_{|G|})$ of $|S| = |G|$ \emph{super-groups}, where each super-group $s_i$ represents the starting values except the ones in group $g_i$. 
%A super group $s$ has the following attributes:
%\begin{compactitem}
    %\item $s.\mathsf{description} = ([x \in \mathsf{Value}, y \in \mathsf{Value}], [x' \in \mathsf{Value}, y' \in \mathsf{Value}])$: This field represents a description of starting values which belong to the super-group $s$. Intuitively, if there exists a starting value $v$ such that $x \leq v \leq y$ or $x' \leq v \leq y'$, then the leader includes $v$ in the super-group $s$. If $S$ is built from $G = (g_1, ..., g_{|G|})$, and we note $[x^j, y^j] \triangleq g_j.\mathsf{description}$, then $s_i.\mathsf{description} = ([x^{1} \in \mathsf{Value}, y^{i-1} \in \mathsf{Value}], [x^{i+1} \in \mathsf{Value}, y^{|G|} \in \mathsf{Value}])$. Of course, 2 values are sufficient for $s_1.\mathsf{description}$ and $s_{|G|}.\mathsf{description}$.  For any value $v$ and any super-group description $\mathit{desc} = ([x, y], [x', y'])$, we define the $\mathsf{match}(v, \mathit{desc}) \in \{\mathit{true}, \mathit{false}\}$ function:
    %\begin{equation*}
        %\mathsf{match}(v, \mathit{desc}) = \mathit{true} \iff x \leq v \leq y \vee x' \leq v \leq y'.
    %\end{equation*}
    
    %\item $s.\mathsf{processes}$: This field denotes the processes whose starting values are included in the group $s$ according to $s.\mathsf{description}$. Formally:
    %\begin{equation*}
    %    s.\mathsf{processes} = \{ P_i \,|\, \mathsf{match}(P_i\text{'s starting value}, s.\mathsf{description}) = \mathit{true}\}.
    % \end{equation*}
    % Moreover, if $G$ is is an array of groups returned by the partition function, then the number of messages confirming the belonging to any super-group $s$ is at least $n-f-t$, and so this number is at least $t+1$ if $f \leq t_{opt} \triangleq c \cdot t$.
%\end{compactitem}

\subsection{Protocol}

In this subsection, we present \textsc{bucket} (\Cref{algorithm:bucket}), a synchronous certification protocol.
We start by giving a description of the protocol.
Then, we perform an analysis which allows us to finalize the protocol details.

\paragraph{Protocol description.}
\textsc{bucket} consists of four synchronous rounds, and it operates in a ``all-to-leader, leader-to-all'' manner.
We explain \textsc{bucket}'s pseudocode (\Cref{algorithm:bucket}) from a perspective of a correct process $P_i$ and the leader.

In the first round, $P_i$ sends its starting value to the leader via a \textsc{disclose} message (line~\ref{line:send_disclose_leader}).
Importantly, $P_i$ sends the $(t+1)$-shared signature of its starting value via the \textsc{disclose} message.

The second round is concerned only with the leader; other processes wait for a leader's message.
There are two possible scenarios which can occur in this round:
\begin{compactitem}
    \item The leader receives the same value $v$ from (at least) $t + 1$ distinct processes (the check at line~\ref{line:t+1_disclose_check}):
    In this case, the leader can combine them to obtain a positive certificate.
    
    \item The leader does not receive the same value from (at least) $t + 1$ distinct processes. In this case, the leader partition the received $\textsc{DISCLOSE}$ messages into a set $G$ of disjoint groups and sends $|G| = O(1)$ $\textsc{PARTITION\_REQ}$ messages to each process, where each $\textsc{PARTITION\_REQ}$ message is associated with a group $g$, such that a process can confirm its starting value does not belong to $g$.
\end{compactitem}

In the third round, $P_i$ share-signs a statement ``My value belongs to $[x,y]$ but not to $g$'' for every $g$ in $G$ such that its starting value is not in $g$, where $x$ (resp. $y$) is be the minimum (resp. maximum) value among the received starting values. The statement is then sent to the leader.

The fourth round is concerned only with the leader; other processes wait for a leader's message. If the leader built a positive certificate in the second round, he broadcasts it. Otherwise, if he received $n-t_{\mathit{opt}}$ $\textsc{PARTITION\_REPLY}$ messages, he builds a negative certificate and broadcasts it.
Upon reception of a valid certificate $\Sigma$, a correct process can trigger $\mathsf{obtain\_certificate}(\Sigma)$.

\subsection{Proof of correctness and complexity}

\begin{lemma}[Safety]
The protocol \name ensures the safety property of certification problem.
\end{lemma}

\begin{proof}
Assume $v \in \mathsf{Value}$ is proposed by every correct process.
Let $(v', \Sigma') \in \mathsf{Value} \times \mathsf{Certificate}$ s.t. a correct process triggered $\mathsf{obtain\_certificate}(v', \Sigma')$. We show that $v=v'$ by contradiction. Let us assume that $v' \neq v$. If $\Sigma'$ is a positive certificate, it means that $v'$ has been share-signed by $t+1$ different processes and so at least by a correct process $P_i$ that would have both (i) share-signed value $v'$ and (ii) started with value $v \neq v'$, which leads to a contradiction. 
If $\Sigma'$ is a negative certificate, by partitioning property, there exists a group $g$ in $\Sigma'$, associated with a $(t+1)$-threshold signature, s.t. $\mathsf{match}(v, g.\mathit{description})$. Thus at least one correct process has both (i) share-signed the description $g.\mathit{description}$ and (ii) started with the value $v$ such that $\mathsf{match}(v, g.\mathit{description})$, which leads to a contradiction.
\end{proof}

\begin{lemma}[Liveness]
The protocol \name ensures the (optimistic) liveness property of certification problem.
\end{lemma}

\begin{proof}
Assume $f \leq \lfloor ct \rfloor$ and the leader $L$ is correct. We will show that every correct process trigger $\mathsf{obtain\_certificate}(v, \Sigma)$ for some $(v, \Sigma) \in \mathsf{Value} \times \mathsf{Certificate}$.
If the leader receives $t+1$ $\textsc{disclose}$ messages with the same value (line \ref{line:t+1_disclose_check}), he can compute a positive certificate (line \ref{line:combine_certification_phase}) that will be broadcast in line \ref{line:bcast_certificate} and received by every correct process in line \ref{line:received_certificate}, allowing each correct process to trigger $\mathsf{obtain\_certificate}()$ in line \ref{line:trigger_obtain_certificate}. Let us assume this is not the case.
Since $f \leq \lfloor ct \rfloor$, it received at least $2t+1$ $\textsc{disclose}$ messages without $(t+1)$ times the same value. Hence, the array $\mathit{groups}$ computed in line is a group-partitioning. Since, by definition, a group $g$ verifies $ |g.\mathit{processes}| \leq t$, $\forall g \in \mathit{groups}, g.\mathit{desc}$ will be signed in line \ref{line:share_sign_description} by every correct process not in $g.\mathit{processes}$, that is by $n-f-t \geq n-\lfloor ct \rfloor - t \geq t+1$ correct processes. Hence, the leader will be able to compute a negative certificate (line \ref{line:compute_negative_certificate}), that will be broadcast in line \ref{line:bcast_certificate} and received by every correct process in line \ref{line:received_certificate}, allowing each correct process to trigger $\mathsf{obtain\_certificate}()$ in line \ref{line:trigger_obtain_certificate}. 
\end{proof}

\begin{lemma}[Termination]
The protocol \name ensures the termination property of certification problem.
\end{lemma}

\begin{proof}
The indication $\mathsf{stop()}$ is triggered at line \ref{line:trigger_stop} anyways.
\end{proof}

\pierre{What about the algorithm \ref{algorithm:bucket_plus} $\textsc{bucket}^{+}$? This algorithm is an extension of $\textsc{bucket}$ with an additional parameter $\Sigma_i$ of type $\mathsf{Certificate}$ for the request $\mathsf{start}()$ ($\Sigma_i = \bot$ is allowed). The idea is that we can note $Oc$ the set of correct processes that invoked $\mathsf{start}()$ with $\Sigma_i \neq \bot$ to represent the set of processes that already obtained a certificate and realize that no messages is exchanged between to correct processes in $Oc$. Thus, if $f \leq t_{\mathit{opt}}$, then in the multi-shot version, the communication complexity of an instance $j'$ with a correct leader following the first instance $j<j'$ with a correct leader, is at most $f$ words (the answers to some at most $f$ fake "AID-REQ" messages).}

\begin{lemma}[$\cert^{+}$ solves certification problem]
Assume that every correct process $P_i$ triggers the request $\mathsf{start}(v_i,v'_i,\Sigma'_i)$ such that (1) $v_i$ is the value proposed by $P_i$, (2) $(v'_i, \Sigma'_i) \neq (\bot, \bot)$ implies that (a) $\Sigma'_i$ is a certificate for value $v'_i$ and (b) if  $v'_i$ has been proposed by every correct process, then $\Sigma'_i$ is a positive certificate for value $v'_i$.
Then, $\cert^{+}$ solves certification problem.
\end{lemma}

\begin{proof}
Safety and termination comes from (i) safety and termination ensured by \cert potentially invoked at line \ref{line:start_Bucket_instance} with a potential indication $\mathsf{obtain\_certificate}(\cdot \; ,\cdot)$ at line \ref{line:obtain_certificate_via_bucket} and (ii) the property (2) in the premises of the lemma.
If the (correct) leader invoked $\cert^{+}.\mathsf{start}(\cdot,\bot,\bot)$, then $\langle \textsc{aid\_req} \rangle$ is broadcast by the leader at line \ref{line:bcast_aid_req} and received by every correct process at line \ref{line:received_aid_req}. Hence, an instance of \cert is started by every correct process at line \ref{line:start_Bucket_instance} and the liveness property comes from the liveness property ensured by \cert with a potential indication $\mathsf{obtain\_certificate}(\cdot \; , \cdot)$ at line \ref{line:obtain_certificate_via_bucket}. Let us assume that the (correct) leader triggered $\cert^{+}.\mathsf{start}(\cdot \;,v',\Sigma')$ with $(v',\Sigma') \neq (\bot, \bot)$. Thus, the leader does not participate to the instance of \cert (line \ref{line:start_Bucket_instance}).
Let $P_j$ be a correct process that triggered $\cert^{+}.\mathsf{start}(\cdot \;,v'_j,\Sigma'_j)$. If $(v'_j,\Sigma'_j) = (\bot, \bot)$, he sends a $\textsc{aid\_req}$ message to the leader at line \ref{line:send_aid_req} that answers with the message $(\textsc{aid\_reply},v',\Sigma')$ at line \ref{line:send_aid_reply}. Thus, process $P_j$ triggers $\mathsf{obtain\_certificate}(v', \Sigma')$ at line \ref{line:obtain_certificate_via_already_obtained_certificate}. By property (2)(a), liveness is ensured.
Assume $(v'_j,\Sigma'_j) \neq (\bot, \bot)$, then process $P_j$ triggers $\mathsf{obtain\_certificate}(v'_j, \Sigma'_j)$ at line \ref{line:obtain_certificate_via_already_obtained_certificate}. By property (2)(a), liveness is ensured.
\end{proof}

\begin{lemma}[$\cert^{+}$ efficiency] \label{lemma:bucket+_efficiency}
Assume that every correct process $P_i$ triggers the request $\mathsf{start}(v_i,v'_i,\Sigma'_i)$ such that (1) $v_i$ is the value proposed by $P_i$, (2) $(v'_i, \Sigma'_i) \neq (\bot, \bot)$ implies that (a) $\Sigma'_i$ is a certificate for value $v'_i$ and (b) if  $v'_i$ has been proposed by every correct process, then $\Sigma'_i$ is a positive certificate for value $v'_i$.
Then, no messages are exchanged between to correct processes $P_i$ and $P_j$ that invoked $\cert^{+}.\mathsf{start}(\cdot \;,v_i',\Sigma'_i)$ and $\cert^{+}.\mathsf{start}(\cdot \;,v_j',\Sigma'_j)$ respectively with $(v_i',\Sigma'_i) \neq (\bot \;, \bot)$ and $(v_j',\Sigma'_j) \neq (\bot \;, \bot)$.
\end{lemma}

\begin{proof}
Let $P_i$ and $P_j$ be two correct processes %that invoked $\cert^{+}.\mathsf{start}(\cdot \;,v_i',\Sigma'_i)$ and $\cert^{+}.\mathsf{start}(\cdot \;,v_j',\Sigma'_j)$ respectively 
s.t. $(v_i',\Sigma'_i) \neq (\bot \;, \bot)$ and $(v_j',\Sigma'_j) \neq (\bot \;, \bot)$. If the leader is not $P_i$ or $P_j$, the result holds anyways. Without loss of generality, let us assume that $P_j$ is the leader. The two processes do not receive a $\textsc{aid\_req}$ message from each other and so both do not communicate in \cert or in $\cert^{+}$.
\end{proof}



\begin{algorithm} [ht]
\caption{\textsc{bucket}: Pseudocode (for process $P_i$)}
\label{algorithm:bucket}
\footnotesize
\begin{algorithmic} [1]

\State \textbf{Variables:}
\State \hskip2em $\mathsf{Value}$ $\mathit{start\_value}_i \gets $ the value for which $P_i$ invoked $\mathsf{start}(\cdot)$
\State \hskip2em $\mathsf{Boolean}$ $\mathit{certificate\_obtained}_i \gets \mathit{false}$ \BlueComment{states whether a positive certificate is obtained}
\State \hskip2em $\mathsf{Certificate}$ $\Sigma_i \gets \bot$ \BlueComment{obtained certificate}
\State \hskip2em $\mathsf{Set}(\mathsf{Group})$ $\mathit{groups}_i \gets \bot$ \BlueComment{partitioning groups; only needed if $P_i$ is the leader}

\medskip
\State \textbf{Constants:}
\State \hskip2em $\mathsf{Integer}$ $t_{\mathit{opt}} = \lfloor c \cdot t \rfloor$
%\State \hskip2em $\mathsf{Integer}$ $\tau = \lceil \max(G) \cdot \frac{2}{c} \rceil$ \BlueComment{number of threshold signature schemes}
%\State \hskip2em $\mathsf{Integer}$ $T_q = \lfloor q \cdot \frac{t}{\tau} \rfloor$, for every $\mathsf{Integer}$ $q \in [1, \tau]$ \BlueComment{thresholds for different threshold signature schemes}


%Sending Phase proposal
% \State \textbf{Constants:}
% %\State $leader \gets \ell$
% \smallskip
% \State \hskip2em $\mathsf{Integer}$ $\tau = \lceil \frac{8}{c} \rceil$ \BlueComment{Number of threshold skims potentially used in the confirm message of Round 3}
% \State \hskip2em $\mathsf{Integer}$ $k_q = \lfloor q\frac{t}{\tau} \rfloor$, for every $q \in [0, \tau]$ \BlueComment{The different threshold of the $\tau$ threshold skims}
% ; $\forall q \in [1:\tau], k_q = q\frac{t}{\tau}$  

\medskip
\State \textbf{Round 1:}
% \smallskip
\State \hskip2em \textcolor{blue}{\(\triangleright\) inform the leader of the starting value}
\State \hskip2em \textbf{send} $\langle \textsc{disclose}, \mathit{start\_value}_i, \mathit{ShareSign}^{t+1}_i(\mathit{start\_value}_i) \rangle$ to the leader \label{line:send_disclose_leader}

\medskip
\State \textbf{Round 2:} \BlueComment{executed only by the leader}
% \smallskip
\State \hskip2em \textbf{if} $P_i$ is the leader:
\State \hskip4em \textbf{if} exists $\mathsf{Value} \text{ } v$ such that $\langle \textsc{disclose}, v, \mathsf{P\_Signature} \text{ } \mathit{sig}\rangle$ is received from $t+1$ processes: \label{line:t+1_disclose_check}
\State \hskip6em \textcolor{blue}{\(\triangleright\) a positive certificate for $v$ can be obtained}
\State \hskip6em $\mathit{certificate\_obtained}_i \gets \mathit{true}$
\State \hskip6em $\Sigma_i \gets \mathit{Combine}^{t + 1}(\{\mathit{sig} \,|\, \mathit{sig} \text{ is received in a } \textsc{disclose} \text{ message}\})$ \label{line:combine_certification_phase}
% \State \hskip4em \textbf{broadcast} $\langle \textsc{certificate}, v, \Psi_v \rangle$ \BlueComment{disseminate the certificate} \label{line:broadcast_certificate_1}

\State \hskip4em \textbf{else:}
\State \hskip6em \textcolor{blue}{\(\triangleright\) a positive certificate cannot be obtained; start partitioning}
\State \hskip6em $\mathit{groups} \gets \mathsf{partition}(\text{received \textsc{disclose} messages})$
%\State \hskip6em $x \gets \text{ the smallest value among \textsc{disclose} messages}$
%\State \hskip6em $y \gets \text{ the biggest value among \textsc{disclose} messages}$

%\State \hskip6em $\mathit{super-groups} \gets \mathsf{allocation}(\text{received \textsc{disclose} messages})$
\State \hskip6em \textbf{for every} $\mathsf{Group}$ $g \in \mathit{groups}$:
%\State \hskip8em \textbf{send} $\langle \textsc{partition\_req}, g.\mathsf{description} \rangle$ to $g.\mathsf{processes}$
\State \hskip8em \textbf{send} $\langle \textsc{partition\_req},  g.\mathsf{description} \rangle$ to all processes except $g.\mathsf{processes}$
%\State \hskip6em \textbf{for every} $\mathsf{SuperGroup}$ $s \in \mathit{super-groups}$:
%\State \hskip8em \textbf{send} $\langle \textsc{partition\_req}, g.\mathsf{description} \rangle$ to $g.\mathsf{processes}$

% \State \hskip4em $(\underline{G}, \underline{D}, J) \gets \mathsf{Partition}(\{\mathit{value} \,|\, \mathit{value} \text{ received in a } \textsc{disclose} \text{ message}\})$
% \State \hskip4em for every $j \in [1, J]$, for every process $P_q$ such that $v_q \in G_j$:
% \State \hskip6em \textbf{send} $\langle \textsc{partition}, D_j \rangle$ to $P_q$ \label{line:send_partition}

\medskip
\State \textbf{Round 3:}
% \smallskip
% \State \hskip2em \textbf{if} a $\langle \textsc{certificate}, v, \Psi_{v}  \rangle$ message is received from the leader:
% \State \hskip4em $\mathit{certificate}_i \gets \Psi_v$ 
% \State \hskip4em \textbf{return} \BlueComment{a certificate for a value is successfully obtained}

%\State \hskip2em \textcolor{blue}{\(\triangleright\) check if the description of the received group matches the starting value}
%\State \hskip2em \textbf{if} $\langle \textsc{partition\_req}, \mathsf{String} \text{ } \mathit{desc} \rangle$ is received from the leader such that $\mathsf{match}(\mathit{start\_value}_i, \mathit{desc})$:
%\State \hskip4em \textcolor{blue}{\(\triangleright\) sign (with all thresholds) the description of the group, and send the signatures back to the leader}
%\State \hskip4em \textbf{send} $\langle \textsc{partition\_reply}, \mathit{desc}, \big[ \mathit{ShareSign}^{T_1}_i(\mathit{desc}), ..., \mathit{ShareSign}^{T_\tau}_i(\mathit{desc}) \big] \rangle$ to the leader

\State \hskip2em \textcolor{blue}{\(\triangleright\) check if the description of the received group excludes the starting value}
\State \hskip2em \textbf{if} $\langle \textsc{partition\_req}, \mathsf{String} \text{ } \mathit{desc} \rangle$ is received from the leader such that $\mathsf{match}(\mathit{start\_value}_i, \mathit{desc}) = \text{false}$:
\State \hskip4em \textcolor{blue}{\(\triangleright\) sign the description of the group, and send the signatures back to the leader}
\State \hskip4em \textbf{send} $\langle \textsc{partition\_reply}, \mathit{ShareSign}^{t+1}_i( \mathit{desc}) \rangle $ to the leader \label{line:share_sign_description}.


\medskip
\State \textbf{Round 4:}
% \smallskip
\State \hskip2em \textbf{if} $P_i$ is the leader:
\State \hskip4em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{false}$:
\State \hskip6em Let $\mathit{replies}$ be the set of received \textsc{partition\_reply} messages
\State \hskip6em \textcolor{blue}{\(\triangleright\) check if enough messages are received for a negative certificate}
\State \hskip6em \textbf{if} $|\mathit{replies}| \geq n - t_{\mathit{opt}}$:
\State \hskip8em $\Sigma_i \gets \mathsf{construct\_negative\_certificate}(\mathit{replies}, \mathit{groups})$ \label{line:compute_negative_certificate}
\State \hskip8em $\mathit{certificate\_obtained}_i \gets \mathit{true}$

\smallskip
\State \hskip4em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{true}$:
\State \hskip6em \textbf{broadcast} $\langle \textsc{certificate}, \Sigma_i \rangle$ \label{line:bcast_certificate} \BlueComment{disseminate the constructed certificate}

\smallskip
\State \hskip2em \textbf{if} $\langle \textsc{certificate}, \mathsf{Certificate} \text{ } \Sigma \rangle$ is received from the leader: \label{line:received_certificate}
\State \hskip4em \textbf{trigger} $\mathsf{obtain\_certificate}(\Sigma)$ \label{line:trigger_obtain_certificate} \BlueComment{attainment of a certificate}
\State \hskip2em \textbf{trigger} $\mathsf{stop}$ \label{line:trigger_stop} \BlueComment{halt certification}


% \State \hskip2em \textbf{if} $|\mathit{ConfirmMessages}| \geq (2+\frac{c}{2})t+1$: 
% \State \hskip4em $\Psi_{\mathit{any}} \gets \mathsf{BuildAllowAnyCertificate}(\mathit{ConfirmMessages}, \underline{D}, J)$
% \State \hskip4em \textbf{broadcast} $\langle \textsc{allow-any}, \Psi_{\mathit{any}} \rangle$ \BlueComment{disseminate the certificate}
 
%  %\State \textbf{if} $Card(ConfirmMessages) \in $ $[2t+1: (2+\frac{c}{2})t+1($
% %\State \hskip2em $\Psi_{ANY} \gets \{\text{received } \textsc{disclose} \text{ messages} \}$ \BlueComment{There is $\frac{c}{2}t = \Theta(t)$ failures, which allows a linear proof}
% %\State \hskip2em \textbf{broadcast} $\langle \textsc{allow-any}, \Psi_{ANY} \rangle_{leader}$

% \State \hskip2em \textbf{else:}
% \State \hskip4em \textbf{return} \BlueComment{There are (at least) $\frac{c}{2}t = \Theta(t)$ failures, which allows a fallback to a quadratic protocol (e.g., \cite{Momose2021})}


% \medskip
% \State \textbf{Round 5:}
% \smallskip
% \State \hskip2em \textbf{if} an $\langle \textsc{allow-any}, \Psi_{\mathit{any}} \rangle$ message is received from the leader:
% \State \hskip4em $\mathit{certificate}_i \gets \Psi_{\mathit{any}}$ \BlueComment{a certificate for any value is  obtained}
% \State \hskip4em \textbf{return}
\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%
% Bucket +
%%%%%%%%%%%%
\begin{algorithm} [ht]
\caption{\textsc{bucket}$^{+}$ : Pseudocode (for process $P_i$)}
\label{algorithm:bucket_plus}
\footnotesize
\begin{algorithmic} [1]
\State \textbf{Variables:}
\State \hskip2em $\mathsf{Value}$ $\mathit{start\_value}_i \gets $ the value $v$ for which $P_i$ invoked $\mathsf{start}(v, v',\Sigma')$
\State \hskip2em $\mathsf{Value}$ $\mathit{certified\_value}_i \gets $ the value $v'$ for which $P_i$ invoked $\mathsf{start}(v,v', \Sigma')$
\State \hskip2em $\mathsf{Certificate}$ $\mathit{certificate}_i \gets $ the certificate $\Sigma'$ for which $P_i$ invoked $\mathsf{start}(v,v', \Sigma')$
\State \hskip2em $\mathsf{Boolean}$ $\mathit{certificate\_obtained}_i \gets $ $(\mathit{certificate}_i \neq \bot )$ \BlueComment{states whether a positive certificate is already obtained}
%\State \hskip2em $\mathsf{Certificate}$ $\Sigma_i \gets \bot$ \BlueComment{obtained certificate}

\medskip
\State \textbf{Round 0:}
% \smallskip
\State \hskip2em \textcolor{blue}{\(\triangleright\) inform if we already have a certificate or not.}
%TO FILL
\State \hskip2em \textbf{if} $\mathit{certificate\_obtained}_i= \mathit{false}$:
\State \hskip4em \textbf{if} $P_i$ \text{is the leader}:
\State \hskip6em \textbf{bcast} $\langle \textsc{aid\_req} \rangle$ \label{line:bcast_aid_req}
\State \hskip4em \textbf{else}:
\State \hskip6em \textbf{send} $\langle \textsc{aid\_req} \rangle$ to the leader \label{line:send_aid_req}

\medskip
\State \textbf{Round 1:}
\State \hskip2em \textbf{if} $\langle \textsc{aid\_req} \rangle$ \text{is received from the leader}: \label{line:received_aid_req}
\State \hskip4em $\mathsf{Bucket}.\mathsf{start}(\mathit{start\_value})$ \label{line:start_Bucket_instance}
\State \hskip2em \textbf{if} $P_i$ \text{is the leader and} $\langle \textsc{aid\_req} \rangle$ \text{is received from process} $P_j$:
\State \hskip4em \textbf{send} $(\textsc{aid\_reply}, \mathit{certified\_value}_i, \mathit{certificate}_i)$ \text{to} $P_j$ \label{line:send_aid_reply}

\medskip
\State \textbf{Round 2:}
\State \hskip2em \textbf{if} $\langle \textsc{aid\_reply}, v', \Sigma' \rangle$ is received from the leader and $\mathit{certificate\_obtained}_i = \mathit{false}$: \label{line:received_aid_reply}
\State \hskip4em
$\mathit{certified\_value}_i \gets v'$, $\mathit{certificate}_i \gets \Sigma'$
%\textbf{trigger} $\mathsf{obtain\_certificate}(v',\Sigma')$

\medskip
\State \textbf{Round 3:}
\State \hskip2em \textbf{pass}

\medskip
\State \textbf{Round 4:}
\State \hskip2em \textbf{upon} $\mathsf{Bucket.obtain\_certificate}(v'', \Sigma'')$:
\State \hskip4em \textbf{if} $\mathit{certificate}_i = \bot$:
\State \hskip6em \textbf{trigger} $\mathsf{obtain\_certificate}(v'', \Sigma'')$ \label{line:obtain_certificate_via_bucket}
\State \hskip2em \textbf{if} $\mathit{certificate}_i \neq \bot$:
\State \hskip4em \textbf{trigger} $\mathsf{obtain\_certificate}(\mathit{certified\_value}_i, \mathit{certificate}_i)$ \label{line:obtain_certificate_via_already_obtained_certificate}
\State \hskip2em \textbf{trigger} $\mathsf{stop}()$
\end{algorithmic}
\end{algorithm}

==> sections/certification.tex <==
% \section{Leader-based certification phase for $n = a\cdot t+1$ with $a=(2+c)$ and $c \in (0,2]$} \label{section:certification}

\section{\core: The Main Building Block of \name} \label{section:certification}

As previously mentioned in \Cref{subsection:fast}, \fast ensures that all correct processes decide if all processes are correct and they propose the same value.
However, if this is not the case, \name needs to employ additional mechanisms in order to solve the Byzantine consensus problem.
In this section, we present \core, the main building block of \name.
\core ensures that, if the actual number of faulty processes $f$ is ``small'', all correct processes decide within (roughly speaking) $f$ rounds, each with an ``all-to-leader, leader-to-all'' communication pattern.

An execution of \core unfolds in \emph{phases}, where each phase has a designated \emph{leader}; the leader of a phase $\phi$ is process $P_{(\phi \text{ } \mathsf{mod} \text{ } n) + 1}$.
In each phase, the leader tries to ensure that all correct processes decide in the ``all-to-leader, leader-to-all'' fashion.
Specifically, the leader has two duties:
\begin{compactenum}
    \item \emph{Certification:} The leader collects the proposed values of all processes, and chooses one value to drive the decision of the system towards.
    However, in order to combat Byzantine leaders, a correct process does not ``accept'' a value suggested by the leader unless the value is accompanied by a proof that the value is ``safe''.
    That is why the leader builds a \emph{constant-sized} proof that the suggested value is safe.
    
    \item \emph{Decision finalization:} Once the leader has built a constant-sized proof of the suggested value, the leader drives the system towards a decision in the HotStuff-like manner.
\end{compactenum}
In this section, we formally describe how the leader of a phase solves both of its aforementioned duties.

\subsection{Certification} \label{subsection:certification}

As already mentioned, the leader of a phase must obtain a constant-sized proof that a value the leader is suggesting can safely be decided, i.e., without fear that the strong validity property could be violated.
Let us consider two scenarios:
\begin{compactitem}
    \item Scenario A (depicted in \Cref{fig:easy_certification}): In this scenario, there are $t + 1$ correct processes that propose the exact same value $v$.
    Hence, when these correct processes inform the leader of their proposals, the leader can combine their partial signatures into a \emph{single} threshold signature proving that (at least) one correct process has proposed $v$.
    Therefore, the leader indeed obtains a constant-sized proof that $v$ is a safe value.
    
    \item Scenario B (depicted in \Cref{fig:easy_certification}): In this scenario, no $t + 1$ correct processes propose the exact same value.
    Therefore, the leader cannot expect to receive $t + 1$ partial signatures of the same value; this is the reason why this scenario is more challenging than Scenario A.
    
    Let us imagine a case where $n = 301$, $t = 100$, and $\mathbb{N}$ is the set of all values processes can propose and decide.
    Moreover, every process is correct and a process $P_i$ proposes value $i$, for every $i \in [1, 301]$.
    In this case, the leader cannot combine the received partial signatures into a threshold signature proving that (at least) $t + 1 = 101$ processes have proposed the same value.
    A straightforward solution for the leader would be to include $t + 2$ received messages into a proof showing that two correct processes have certainly proposed different values.
    However, this proof would be of size $O(t)$, which means that the entire phase would ``suffer'' from quadratic communication as the leader will broadcast a message of size $O(t)$; recall that, if there are no faulty processes, we aim to keep the communication complexity of \name linear (and not $O(n \cdot t)$).
\end{compactitem}

% It already exists a solution, based on a rotating leader, for a weakest variant \cite{Cohen2022} where strong validity is replaced by weak validity that only ensures that: If all processes are correct, then a value decided by a process was previously proposed. The  challenge is to prove with a constant-sized message that a value can be decided without fear of strong validity violation. In the simple scenario $A$ (see figure \ref{fig:easy_certification}) where at least $t+1$ processes  propose the same value $v^{*}$ with a $(t+1,n)$ partial signature, the leader can combine partial signatures to obtain a constant-sized $(t+1,n)$ threshold signature for value $v^{*}$, broadcast it and hence convince every process that at least, one correct process proposed $v^{*}$, which means it is safe to decide $v^{*}$.

\begin{figure}%
    \centering
    \subfloat[\centering More than $t+1$ processes proposed $v^{*}$. ]{{\includegraphics[width=7cm]{figures/AscenarioDisclose.png} }}%
    \qquad
    \subfloat[\centering A $(t+1,n)$ threshold signature is enough to ensure deciding $v^{*}$ cannot violate strong validity. ]{{\includegraphics[width=7cm]{figures/EasyCertification.png} }}%
    \caption{Easy Certification}%
    \label{fig:easy_certification}%
\end{figure}




% But in more difficult scenario $B$ (see figure \ref{fig:hard_certification}) where there is no subset of $t+1$ processes that proposed the same value, the previous strategy does not work anymore. Let us imagine we want to solve the problem for $n = 301$, $t=100$ and $\mathbb{N}$ as set of possible inputs. What if the leader receives the integers $1,2,..., n$ ? A naive solution would be concatenating $t+2$ signatures to prove that there are at least two correct processes that proposed  different values. But such a solution implies a message containing $O(t)$ signatures which tackles adaptiveness.

\begin{figure}%
    \centering
    \subfloat[\centering scattered proposals]{{\includegraphics[width=7cm]{figures/BscenarioDisclose.png} }}%
    \qquad
    \subfloat[\centering proof of validity with $O(t)$ signatures]{{\includegraphics[width=7cm]{figures/HardCertification.png} }}%
    \caption{Hard Certification}%
    \label{fig:hard_certification}%
\end{figure}

\smallskip
\noindent \textbf{Constant-sized validity proofs.}
The goal of the leader of a phase is to obtain a locally-verifiable, constant-sized cryptographic proof $\Psi_v$ vouching that value $v$ is \emph{valid}.
Moreover, in the case in which all correct processes propose $v$, it is impossible for any (either correct or faulty) process to obtain such a cryptographic proof for a value different from $v$:
\begin{compactitem}
    \item \emph{Computability:} If all correct processes propose $v$ to \name, then no process (even if faulty) obtains $\Psi_{v'}$ for a value $v' \neq v$.
\end{compactitem}
If we could implement such a cryptographic primitive, then the protocol of \cite{Cohen2022} could be modified in the following manner in order to satisfy strong validity:
\begin{compactitem}
    \item A correct leader accompanies each value by a cryptographic proof that the value is valid.
    
    \item A correct process ignores any value not accompanied by a proof that the value is valid.
\end{compactitem}
Suppose that all correct processes propose the same value $v$ and that a correct process $P_i$ decides $v'$ from \name.
Given that $P_i$ ignores values not accompanied by a proof, $P_i$ has obtained $\Psi_{v'}$ before deciding.
The computability property of the cryptographic primitive guarantees that $v' = v$, implying that strong validity is satisfied.
Given that the proof is of constant size, the communication complexity of the modified version of \cite{Cohen2022} remains $O(n \cdot f)$, where $f$ is the actual number of faulty processes.

Hence, the challenge is to compute such a proof in a leader-based (and ``adaptive'') fashion, avoiding the quadratic communication complexity of the ``all-to-all'' communication pattern. 

\smallskip
\noindent \textbf{The Partition-based certificate}

Since the scenario A is straightforward, we focus on the scenario B. Let us assume a leader suggesting a value $v$ with an associated certificate $\Psi_{v}$. Proving that deciding $v$ does not violate strong validity is equivalent to prove that either 
\begin{itemize}
    \item $(C_1)$ It does not exists another value $v' \neq v$ proposed by all correct processes, or
    \item $(C_2)$ Two correct processes proposed two different values
\end{itemize}

In this paper, a correct leader will face scenario B by partitioning the received proposals into multisets $G_1, ..., G_{|J|}$.
Then, he will ask each replica to confirm that its proposal is indeed in the corresponding partition $G_j$ for some $j$ (we note $D_j$ the description of $G_j$).
Finally, he will suggest a value $v$ with an attached constant-sized \emph{partition-certificate} $\Psi_{v}$ with a family $((D_j,TS^{s_j}(D_j)))_{j \in J}$, where $TS^{s_j}(D_j)$ is a $(s_j,n)$-threshold signature of description $D_j$ of group $G_j$. Intuitively, the number $s_j$ represents a number of voters for some values in a common group $G_j$.
This partition-certificate will verify the \emph{partition-condition}, i.e. the disjunction of one of the following key conditions:
\begin{itemize}
    \item $\forall j^{*} \in J$, $\sum_{j \in J \setminus \{j^{*}\}} s_j > t$
    \item $\exists j_v \in J, G_{j_v} = \{ v\}$ and $\forall j^{*} \in J \setminus{\{j_v\}}$, $\sum_{j \in J \setminus \{j^{*}\}} s_j > t$
\end{itemize}

We give an intuition of this two predicates:

\begin{itemize}
    \item The first predicate clearly implies $C_2$. Indeed, let us assume the opposite. Then there exists a value $v_{j^{*}}$ in a group $G_{j^{*}}$ proposed by all correct processes, while all the other "votes" are from Byzantine processes. But this is impossible, since $\forall j^{*} \in J$, $\sum_{j \in J \setminus \{j^{*}\}} s_j > t$. 
    
\item The second predicate clearly implies ($C_1$ or $C_2$). Indeed, let us assume the opposite. Then there exists a value $v_{j^{*}}$, different from $v$ in a group $G_{j^{*}}$ for some $j^{*} \neq j_v$ proposed by all correct processes, while all the other "votes" are from Byzantine processes. Let us remark that if $\sum_{j \in J \setminus \{j_v\}} s_j \leq t$, it is not problematic, because $v \in G_{j_v} = \{v\}$ is the value suggested by the leader and so $C_1$ is not questioned.
\end{itemize}

The key part of our algorithm enables to build a partition of the proposals to then compute a partition-certificate verifying the partition-condition.

\smallskip
\noindent \textbf{The skeleton of a view-protocol}

TO DO: write the skeleton of the algorithm without providing any details of how the partitition is computed

\smallskip
\noindent \textbf{The partitioning}

Let us consider scenario B where in which the leader does not collect $t+1$ identical values.

In this case, the leader can partition the received values $V$ into $|J|$ groups $G_j$, for every $j \in J$, in the following manner:
\begin{compactenum}
\item $\#(G_1) \leq ... \leq \#(G_{|J|}) $; a
\item $\forall j \in [1, J]: \#(G_j) \leq t$;
\label{item:star}
\item $\forall (i,j) \in [1, J]^2: \#(G_i) + \#(G_j) > t $ 
\label{item:pair-lower-than-t} (a pair that does not satisfy this predicate can be merged into a new one that satisfies the second property); and
\item 
\begin{compactitem}
    \item $J \geq 3$ if $\#(V) \geq 2t+1$ (\Cref{lemma:lower_bound_size_of_partition} formally proves this claim); and 
    
    \item $J$ $\leq \lceil 2a \rceil - 1$ (\Cref{lemma:upper_bound_size_of_partition} formally proves this claim).
\end{compactitem}
\end{compactenum}

We now present a few intermediate results.

\begin{lemma}\label{lemma:lower_bound_multiplicity_of_sub_partition}
Let $(G_{j})_{j \in [1, J]}$ be a partition of a set of values  such that (1) $J \geq 2$, and (2) $\forall j,j' \in [1, J], \#(G_j)+\#(G_{j'}) \geq t+1$.
Then, for every $k \geq 2$ and every sequence $j_1, ..., j_k \in [1, J]$,
$\#(G_{j_1})+\#(G_{j_2})+...+\#(G_{j_k}) \geq k \frac{(t+1)}{2}$.
\end{lemma}

\begin{proof}
Without loss of generality, let $\#(G_1) \leq ... \leq \#(G_{J})$.
Since $\#(G_1) \leq \#(G_2)$ and $\#(G_1) + \#(G_2) \leq t + 1$, we have that $\#(G_2) \leq \frac{t + 1}{2}$.
Therefore, for every $j > 1$, $\#(G_j) \geq \frac{t + 1}{2}$.

Finally, $\#(G_{j_1})+\#(G_{j_2})+...+\#(G_{j_k}) = \big(\#(G_{j_1}) + \#(G_{j_2})\big) + \#(G_{j_3}) + ... + \#(G_{j_k}) \geq (t + 1) + (k - 2)\frac{t + 1}{2} = 2\frac{t + 1}{2} + (k - 2)\frac{t + 1}{2} = \frac{t + 1}{2}(2 + k - 2) = k\frac{t + 1}{2}$.
Hence, the lemma holds.
\end{proof}

\begin{lemma}\label{lemma:lower_bound_size_of_partition}
Let $(G_{j})_{j \in [1, J]}$ be a partition of a set of values $V$ with $\#(V) \geq 2t+1$ such that $\forall j \in [1, J], \#(G_j) \leq t$.
Then, $J \geq 3$.
\end{lemma}
\begin{proof}
We assume that, by contradiction, $J \leq 2$.
Then, $\#(V) \leq 2t$, which contradicts the fact that $\#(V) \geq 2t + 1$.
Thus, the lemma holds.
\end{proof}

\begin{lemma}\label{lemma:upper_bound_size_of_partition}
Let $(G_{j})_{j \in [1, J]}$ be a partition of a set of values $V$ with $\#(V) \leq n = at+1$ such that (1) $a \geq 2$, (2) $\forall j,j' \in [1, J], \#(G_j)+\#(G_{j'}) \geq t+1$, and (3) $\forall j \in [1, J], \#(G_j) \leq t$.
Then, $J \leq \lceil 2a \rceil -1$.
\end{lemma}

\begin{proof}
Without loss of generality, let $\#(V) = n = at + 1$.
By \Cref{lemma:lower_bound_size_of_partition}, we have $J \geq 3$.
By \Cref{lemma:lower_bound_multiplicity_of_sub_partition}, we have $\#(V) \geq \frac{J}{2}(t + 1)$.

By contradiction, let $J \geq \lceil 2a \rceil$.
Hence, $\#(V) \geq \frac{\lceil 2a \rceil}{2}(t + 1) \geq a(t + 1)$.
For every $a \geq 2$, we have $a(t + 1) > at + 1$, which contradicts $\#(V) = n$.
Therefore, the lemma holds.
\end{proof}

\begin{lemma}\label{lemma:precision}
Let the leader receive $z_j \leq t$ well-formed \textsc{confirm} messages with $\tau$ partial signatures for group $G_j$: $\mathit{PS}^{\lfloor \frac{t}{\tau} \rfloor}, \mathit{PS}^{2\lfloor \frac{t}{\tau} \rfloor}, ..., \mathit{PS}^{\tau \lfloor \frac{t}{\tau} \rfloor}$. 
Then, the leader can compute a $(s_j,n)$-threshold signature for group $G_j$  with $z_j - s_j \leq  \lfloor \frac{t}{\tau} \rfloor - 1$.
%with $s_j \geq z_j - \lfloor \frac{t}{\tau} \rfloor + 1$.
\end{lemma}

\begin{proof}
The Euclidian division of $z_j$ by $\frac{t}{\tau}$ gives
$z_j = x_z \lfloor \frac{t}{\tau} \rfloor + y_z $ with $y_z \in [0, \lfloor \frac{t}{\tau} \rfloor-1]$ and $x_z \in [0, \tau]$.
Hence, the leader can combine $x_z \lfloor \frac{t}{\tau} \rfloor$ $(x_z \lfloor \frac{t}{\tau} \rfloor,n)$-partial signatures to obtain an $(x_z\lfloor \frac{t}{\tau} \rfloor,n)$-threshold signature. Finally, $z_j - x_z \lfloor \frac{t}{\tau} \rfloor = y_z \leq \lfloor \frac{t}{\tau} \rfloor-1$, which concludes the proof.

\end{proof}

\smallskip
\noindent \textbf{Ensuring partition-condition in the trivial case $|J| \geq 4$.}

In this situation, the leader can suggest any value $v$.
First, recall that, for every $j, j' \in J$, $\#(G_j) + \#(G_{j'}) > t$.
%Hence, at most one group can ``completely'' be Byzantine.
%Therefore, we are left with (at least) three groups that contain a correct process. Thus the idea is to provide a certificate with $|J|$ threshold-signatures, whose thresholds $(s_j)_{j \in J}$ verify: $\forall j^* \in J$, $\sum\limits_{j \in J \setminus{\{j^*\}}} s_j \geq t+1$. Hence, there is no way that the provider of such a certificate, "hide" a value $v_{j^*}$ (in a multiset $G_{j^*}$ for some $j^* \in J$)  that would be the unique value proposed by correct processes.  

Let $j^* \in J$.
Then, $\sum\limits_{j \in J \setminus{\{j^*\}}} z_j \geq (|J|-1)\frac{t + 1}{2}  + (|J|-1)$ (by \Cref{lemma:lower_bound_multiplicity_of_sub_partition}).
Furthermore, $\sum\limits_{j \in J \setminus{\{j^*\}}} (z_j) > (|J|-1)\frac{t + 1}{2} - (|J|-1)\frac{t}{\tau} > (|J|-1)\frac{t + 1}{2} - (|J|-1)\frac{t + 1}{\tau}$.
Finally, we need to ensure that $(|J|-1)\frac{t + 1}{2} - (|J|-1)\frac{t + 1}{\tau} \geq t + 1$, which is ensured for $\tau \geq 6$.
Hence, if $|J| \geq 4$, it suffices for $\tau$ to be equal to $6$ to satisfy partition-condition.

\smallskip
\noindent \textbf{A solution to the case of $|J| = 3$, with $\frac{4}{c}$ threshold skims.}

First if $f >\frac{ct}{2}$, the number of Byzantine processes is linear and so a fallback is enough to ensure adaptiveness.

Let us assume $f \leq \frac{ct}{2}$.

We have $\#(G_1) + \#(G_2) + \#(G_3) = \#(V) \geq 2t+1 + \frac{ct}{2}$ and $\#(G_3) \leq t$.
In that case, the leader propose any value. Since $\#(G_1) + \#(G_2) = \#(V) - \#(G_3) \geq 2t+1 + \frac{ct}{2} -t \geq t+1 + \frac{ct}{2}$ and $\forall j^{*} \in J$, $\sum_{j \in J\setminus \{j^*\}} \#(G_j) \geq \#(G_1) + \#(G_2)$, we have $\forall j^{*} \in J$, $\sum_{j \in J \setminus{\{j^{*}\}}} z_j \geq t+1 + \frac{ct}{2}$ and so $\forall j^{*} \in J$, $\sum_{j \in J \setminus{\{j^{*}\}}} s_j \geq t+1 + \frac{ct}{2} - 2\frac{t}{\tau}$. Thus $\tau \geq \frac{4}{c}$ is enough to ensure partition-condition $\sum_{j \in J \setminus{\{j^{*}\}}} s_j \geq t+1$.

\smallskip
\noindent \textbf{The problem of case $|J| = 3$: Why cannot we use a number of threshold skims independent from $c$.}

This case is more problematic. Indeed, even with $\#(V) \geq 2t+\frac{c}{2}t+1$, it is impossible to avoid the scenario $G_i=\{w_i\}$, for each $i \in \{1,2,3\}$ with $\#(G_1) = \frac{c}{2}t + 1 + 2 \epsilon$ and $\#(G_2) = \#(G_3) = t- \epsilon$.
In that case it is impossible to propose $v = w_{j_v}$ for some $j_v$ such that $\forall j^{*} \in J \setminus \{j_v\}$, $\sum_{ j \in J\setminus \{j^{*}\}} z_j > t + 1 + \epsilon + \frac{c}{2}t$. Thus $\sum_{ j \in J\setminus \{j^{*}\}} s_j > t + 1 + \epsilon + \frac{c}{2}t - 2\frac{t}{\tau}$ is also impossible to ensure. 
Hence, there is always a scenario where the number of threshold skims is equal to $\frac{4}{c}$, which is problematic if $c$ is very low.
An alternative would be sigma compressed signature, since the threshold can be decided in the run. But a logarithmic term has to be added, i.e. the size of the certificate would be a $\Theta(log(n))$.

\smallskip
\noindent \textbf{A few examples}

\begin{itemize}
    \item Case $c=2$, i.e. $n=4t+1$.
    In that case,  $\#(V) \geq 3t+1$ and so necessarily, $|J| \geq 4$ which means the trivial solution for $|J| \geq 4$ can be applied without any fall-back.
    
    \item Case $c=1$, i.e. $n=3t+1$. In that case, if $|J|=3$, and $f \geq n/6$, a fallback can be performed. If, $f \leq n/6$, then the certificate will contain only $4$ threshold signatures. 

\item Case $c=0.5$, i.e. $n=2.5t+1$.
In that case, if $|J|=3$, and $f \geq n/5$, a fallback can be performed. If, $f \leq n/5$, then the certificate will contain only $8$ threshold signatures. 

\item Case $c=0.1$, i.e. $n=2.1t+1$.
In that case, if $|J|=3$, and $f \geq n/42$, a fallback can be performed. If, $f \leq n/42$, then the certificate will contain $40$ threshold signatures.
This example shows the limit of the solution for a small constant $c$.
\end{itemize}


\smallskip
\noindent \textbf{Attainment of constant-sized validity proofs.}
We now present a protocol (\Cref{algorithm:certification_phase}) with linear communication complexity and constant latency 
that ensures (1) computability (even if the leader is Byzantine and $t$ failures occur), and (2) if the leader is correct and  $f \leq \frac{c}{2}t$ failures occur,\footnote{Recall that $c = \Omega(1)$ is a fixed constant and $f \leq t$ is the actual number of faulty processes.} every correct process receives a cryptographic proof $\Psi_v$ vouching that some value $v$ is valid.
The spirit of \Cref{algorithm:certification_phase} is captured by figure \Cref{fig:partitioning_certification}.
We separate the protocol into rounds:

\begin{figure}%
    \centering
    \subfloat[\centering scattered proposals]{{\includegraphics[width=7cm]{figures/CscenarioDisclose.png} }}%
    \qquad
    \subfloat[\centering Request for partial-signature for belonging to one set of the partition ]{{\includegraphics[width=7cm]{figures/Partitioning.png} }}%
    \qquad
    \subfloat[\centering  for each set $G_j$ of the partition, $z_j$ processes send partial-signature to confirm their values belong $G_j$  ]{{\includegraphics[width=7cm]{figures/ConfirmationPartition.png} }}%
    \qquad
    \subfloat[\centering  proof of validity with 5 $(k_j,n)$-threshold signatures, with $0 \leq z_j-k_j \leq \frac{c}{10}t $ ]{{\includegraphics[width=7cm]{figures/constantCertificate.png} }}%
    \caption{Partitioning-based Certification. For $a \in (2,3]$ (i.e. $c \in (0,1]$), they are at most 5 subsets in the partition}%
    \label{fig:partitioning_certification}%
\end{figure}

\begin{algorithm} [ht]
\caption{Certification: Pseudocode for process $P_i$}
\label{algorithm:certification_phase}
\begin{algorithmic} [1]

%Sending Phase proposal
\State \textbf{Constants:}
%\State $leader \gets \ell$
\smallskip
\State \hskip2em $\mathsf{Integer}$ $\tau = \lceil \frac{8}{c} \rceil$ \BlueComment{Number of threshold skims potentially used in the confirm message of Round 3}
\State \hskip2em $\mathsf{Integer}$ $k_q = \lfloor q\frac{t}{\tau} \rfloor$, for every $q \in [0, \tau]$ \BlueComment{The different threshold of the $\tau$ threshold skims}
% ; $\forall q \in [1:\tau], k_q = q\frac{t}{\tau}$  

\medskip
\State \textbf{Round 1:} \label{line:certification_phase_start}
\smallskip
\State \hskip2em \textbf{send} $\langle \textsc{disclose}, v_i, \mathit{ShareSign}^{t+1}_i(\mathit{proposal}_i) \rangle$ to the leader \label{line:send_disclose_1}

\medskip
\State \textbf{Round 2:} (if $P_i$ is the leader)
\smallskip
\State \hskip2em \textbf{if} exists $\mathsf{Value} \text{ } v$ such that $\langle \textsc{disclose}, v, \mathsf{P\_Signature} \text{ } \mathit{sig}\rangle$ is received from $t+1$ processes: \label{line:t+1_disclose}
\State \hskip4em \textcolor{blue}{\(\triangleright\) a certificate for $v$ is obtained}
\State \hskip4em $\mathsf{Certificate} \text{ } \Psi_v \gets \mathit{Combine}^{t + 1}(\{\mathit{sig} \,|\, \mathit{sig} \text{ is received in a } \textsc{disclose} \text{ message}\})$ \label{line:combine_certification_phase}
\State \hskip4em \textbf{broadcast} $\langle \textsc{certificate}, v, \Psi_v \rangle$ \BlueComment{disseminate the certificate} \label{line:broadcast_certificate_1}

\State \hskip2em \textbf{else:}
\State \hskip4em $(\underline{G}, \underline{D}, J) \gets \mathsf{Partition}(\{\mathit{value} \,|\, \mathit{value} \text{ received in a } \textsc{disclose} \text{ message}\})$
\State \hskip4em for every $j \in [1, J]$, for every process $P_q$ such that $v_q \in G_j$:
\State \hskip6em \textbf{send} $\langle \textsc{partition}, D_j \rangle$ to $P_q$ \label{line:send_partition}

\medskip
\State \textbf{Round 3:}
\smallskip
\State \hskip2em \textbf{if} a $\langle \textsc{certificate}, v, \Psi_{v}  \rangle$ message is received from the leader:
\State \hskip4em $\mathit{certificate}_i \gets \Psi_v$ 
\State \hskip4em \textbf{return} \BlueComment{a certificate for a value is successfully obtained}
\State \hskip2em \textbf{if} a $\langle \textsc{partition}, D \rangle$ message is received from the leader such that $\mathsf{Match}(v_i, D)$: \label{line:receive_partition}
\State \hskip4em \textbf{send} $\langle \textsc{confirm}, D, [\mathit{ShareSign}^{k_1}_i(D), ..., \mathit{ShareSign}^{k_\tau}_i(D)] \rangle$ to the leader \label{line:send_confirm}

\medskip
\State \textbf{Round 4:} (if $P_i$ is the leader)
\smallskip
\State \hskip2em Let $\mathit{ConfirmMessages}$ be the set of well-formed received \textsc{confirm} messages \label{line:confirm_messages}

\State \hskip2em \textbf{if} $|\mathit{ConfirmMessages}| \geq (2+\frac{c}{2})t+1$: 
\State \hskip4em $\Psi_{\mathit{any}} \gets \mathsf{BuildAllowAnyCertificate}(\mathit{ConfirmMessages}, \underline{D}, J)$
\State \hskip4em \textbf{broadcast} $\langle \textsc{allow-any}, \Psi_{\mathit{any}} \rangle$ \BlueComment{disseminate the certificate}
 
 %\State \textbf{if} $Card(ConfirmMessages) \in $ $[2t+1: (2+\frac{c}{2})t+1($
%\State \hskip2em $\Psi_{ANY} \gets \{\text{received } \textsc{disclose} \text{ messages} \}$ \BlueComment{There is $\frac{c}{2}t = \Theta(t)$ failures, which allows a linear proof}
%\State \hskip2em \textbf{broadcast} $\langle \textsc{allow-any}, \Psi_{ANY} \rangle_{leader}$

\State \hskip2em \textbf{else:}
\State \hskip4em \textbf{return} \BlueComment{There are (at least) $\frac{c}{2}t = \Theta(t)$ failures, which allows a fallback to a quadratic protocol (e.g., \cite{Momose2021})}


\medskip
\State \textbf{Round 5:}
\smallskip
\State \hskip2em \textbf{if} an $\langle \textsc{allow-any}, \Psi_{\mathit{any}} \rangle$ message is received from the leader:
\State \hskip4em $\mathit{certificate}_i \gets \Psi_{\mathit{any}}$ \BlueComment{a certificate for any value is  obtained}
\State \hskip4em \textbf{return}
\end{algorithmic}
\end{algorithm}

\begin{algorithm} [ht]
\caption{Helper functions: Pseudocode for process $P_i$}
\label{algorithm:helper_functions}
\begin{algorithmic} [2]
\State \textbf{Precondition} $\nexists W \subseteq Values$, s.t. $\forall v, v' \in W$, $v=v'$ $\wedge$ $\#(W) = 2t+1$ %$|W| = 2t+1$
\State \textbf{function} $\mathsf{PrePartition}(Values)$:

\State \hskip2em $y \gets 1$, $H_1 \gets \{\}$, $\mathit{partition} = []$
\State \hskip2em $values = [w^1,...,w^{|Values|}]$, where $Values = \bigcup_{i \in [1:|Values|]} w^i \wedge w^1 \prec ... \prec w^{|Values|}$ where $\prec$ is an arbitrary order.
\State \hskip2em \textbf{for} $i \in [1: |Values|]$:
\State \hskip4em \textbf{if} $\#(H_y) + \#(\{w^i\}) \leq t+1$:
\State \hskip6em $H_y \gets H_y \cup \{w^i\}$
\State \hskip4em \textbf{else}:
\State \hskip6em $partition.add(H_y)$
\State \hskip6em $y \gets y+1$
\State \hskip6em $H_y = \{w^i\}$

\State \textbf{Postcondition}
$(H_j)_{j \in J'}$ is a partition of $Values$ such that:
\begin{enumerate}
\item $\forall x \in [1:\lfloor |J'|/2 \rfloor]$, $\#(H_{2x-1}) + \#(H_{2x}) \geq t+1$
\item $\forall j \in J'$,  $\#(H_j) \leq t$  
\item $|J'| \leq 2a+1$
\end{enumerate}


\smallskip \smallskip
\State \textbf{Precondition} Postcondition of $\mathsf{PrePartition}$
\State \textbf{function} $\mathsf{PostPartition}([H_1, ..., H_{|J'|}])$
\State \hskip2em \textbf{initially}
\State \hskip2em $\mathcal{H} = \{H_1, ..., H_{|J'|} \}$
\State \hskip2em $description : H \in \mathcal{H} \mapsto [[w^a, w^b]]$ s.t. $\forall w \in H$, $w^a \preceq w \preceq w^b$.
\State \hskip2em \textbf{while}(true):
\State \hskip4em $H_a \gets arg \; min_{H_j \in \mathcal{H}} \#(H_j)$ 
\State \hskip4em $H_b \gets arg \; min_{H_j \in \mathcal{H} \setminus{\{H_a\}}} \#(H_j)$
\State \hskip4em \textbf{if}: $\#(H_a) + \#(H_b) \geq t+1$
\State \hskip6em \textbf{exit}
\State \hskip4em \textbf{else}:
\State \hskip6em $H_c \gets H_a \cup H_b$
\State \hskip6em $description(H_c) \gets concatenate(description(H_a), description(H_b))$
\State \hskip6em $\mathcal{H} \gets ((\mathcal{H} \setminus{\{H_a\}}) \setminus{\{H_b\}}) \cup \{ H_c\}$
\State \hskip2em $(G_j)_{j \in J} \gets \mathcal{H}$ \text{ with } $\#(G_1) \leq ... \leq \#(G_{|J|}) $
\State \hskip2em $(D_j)_{j \in J} \gets (description(G_j)_{j \in J})$

\State \hskip2em \textbf{return} $((G_j)_{j \in J}, (D_j)_{j \in J}, J)$

\State \textbf{Postcondition}
$(G_j)_{j \in J}$ is a partition of $Values$ such that:
\begin{enumerate}
\item $\#(G_1) \leq ... \leq \#(G_{|J|}) $ by construction 
\item $\forall j \in [1:|J|]$,  $\#(G_j) \leq t$ 
\item $\forall (i,j) \in J^2$,  $\#(G_i) + \#(G_j) > t $  
\label{item:pair-lower-than-t}.
\item 
\begin{itemize}
    \item $|J|$ $\geq 2+\lfloor \frac{c}{2}+1\rfloor$
    
    \item $|J|$ $\leq \left\{
    \begin{array}{ll}
        \lceil 2 a \rceil & \mbox{if } (c - \lfloor c \rfloor ) \in (0,0.5] \\
        \lfloor 2 a \rfloor & \mbox{if } (c - \lfloor c \rfloor ) \in (0.5,1) \\
         2 a - 1  & \mbox{if } c \in \mathbb{N}^{>0}
    \end{array}
\right.$
\end{itemize}
\end{enumerate}

\smallskip \smallskip

\State \textbf{Precondition} $\nexists W \subseteq Values$, s.t. $\forall v, v' \in W$, $v=v'$ $\wedge$ $|W| = 2t+1$
\State \textbf{function} $\mathsf{Partition}(Values)$:
\State \hskip4em \textbf{return} $\mathsf{PostPartition}$ $(\mathsf{PrePartition}(Values))$
\smallskip \smallskip


\State \textbf{function} $\mathsf{Match}(v,[[w^a_1,w^b_1], ..., [w^a_x,w^b_x]])$:
\State \hskip2em \textbf{return}  $\exists q \in [1:x]$ s.t. $w^a_q \preceq v \preceq w^b_q$.

\smallskip
\smallskip

\State \textbf{Precondition} $|ConfirmMessages| \geq 2t+\frac{c}{2}+1$
\State \textbf{function} $\mathsf{BuildAllowAnyCertificate}(ConfirmMessages, (D_j)_{j \in J}, J)$:
\State \hskip2em \textbf{for} $j \in J$:
\State \hskip4em
$z_j \gets Card(\{msg | \text{in } ConfirmMessages \text{ for description } D_j \})$
\State \hskip4em $k_j \gets max(\{k | k \in \{k_1,...,k_{\tau}\} \wedge k \leq z_j \})$,
\State \hskip4em  $\sigma^j \gets \mathit{Combine}^{k_j}(\{\mathit{sig} \,|\, \mathit{sig} \text{ received in } \text{in } ConfirmMessages \text{ for description } D_j \})$
\State \hskip2em \textbf{return} $ [\sigma^1, ..., \sigma^{|J|}]$
\State \textbf{Postcondition} $\sum_{j \in J} k_j \geq 2t+1$
\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%

\smallskip
\noindent \textit{First and second rounds (i.e., \textsc{disclose} and \textsc{partition} rounds).}
Every process $P_i$ sends a \textsc{disclose} message containing its proposal $v_i$ and the $(t+1,n)$-partial signature $\mathit{ShareSign}^{t+1}_i(v_i)$ to the leader (line~\ref{line:send_disclose_1}).
The leader receives a multiset $(V,m)$ of values, where $V$ is the set of different values and $m(v\in V) \in \mathbb{N}$ is the multiplicity of value $v \in V$. Moreover, $\#(V) \triangleq \sum\limits_{v \in V}m(v) \in [n-f,n]$.  
If the leader is correct and receives $t+1$ times the same value $v^{*}$ (line~\ref{line:t+1_disclose}),  then it can compute a threshold signature $\mathit{TS}^{t+1}(v^{*})$ for $v^{*}$ proving that (at least) one correct process proposed $v^{*}$ (line~\ref{line:combine_certification_phase}).
Importantly, this shows that deciding $v^{*}$ would not violate strong validity, i.e., $v^*$ is safe.
As already mentioned, such a scenario is easily solvable (and depicted in \Cref{fig:easy_certification}).

Therefore, we consider the other case in which the leader does not collect $t + 1$ identical values (recall that \Cref{fig:hard_certification} depicts this case); we name this scenario ``hard certification''.
In this case, the leader can partition the received values $V$ into $J$ groups $G_j$, for every $j \in [1,  J]$, in the following manner:
\begin{compactenum}
\item $\#(G_1) \leq ... \leq \#(G_{J}) $; and %$|G_1| \leq ... \leq |G_{|J|}| $ by construction
\item $\forall j \in [1, J]: \#(G_j) \leq t$; and %$|G_j| \leq t$ (by (*))
\label{item:star}
\item $\forall (i,j) \in [1, J]^2: \#(G_i) + \#(G_j) > t $  %$|G_i| + |G_j| > t $ 
\label{item:pair-lower-than-t} (a pair that does not satisfy this predicate can be merged into a new one that satisfies the second property); and
\item 
\begin{compactitem}
    \item $J \geq 3$ (\Cref{lemma:lower_bound_size_of_partition} formally proves this claim); and 
    
    \item $J$ $\leq \lceil 2a \rceil - 1$ (\Cref{lemma:upper_bound_size_of_partition} formally proves this claim).
\end{compactitem}
% The lower bound comes from property \ref{item:star} and the fact we assume $n-f> 2t$ (since $f \leq \frac{c}{2}t$) in the optimistic case when no fallback is needed. The upper bound comes from property \ref{item:pair-lower-than-t}.
\end{compactenum}

For every $j \in [1, J]$, the leader sends the \textsc{partition} message to all processes whose values belong to $G_j$ (line~\ref{line:send_partition}).

\smallskip
\noindent \textit{Third and fourth rounds (i.e., \textsc{confirm} rounds).}
Once a correct process receives a \textsc{partition} message describing a corresponding group (line~\ref{line:receive_partition}), the process sends a \textsc{confirm} message containing $\tau$ different partial signatures of the description of the received group (line~\ref{line:send_confirm}); there are $\tau$ different thresholds, i.e., for every $q \in [1, \tau]$, a corresponding threshold is $\lfloor \frac{q \cdot t}{\tau} \rfloor$.

\smallskip
\noindent \textit{Fifth round (i.e., \textsc{allow-any} round)}.
For each $j \in [1, J]$, the leader receives $z_j$ (well-formed) CONFIRM messages (from correct or faulty processes) with a partially-signed description $D_j$ of group $G_j$ (line~\ref{line:confirm_messages}).
For every $j \in [1, J]$, there exists $q_j \in [0, \tau]$ such that $z_j \in [q_j\lfloor \frac{t}{\tau} \rfloor, (q_j + 1)\lfloor \frac{t}{\tau} \rfloor - 1]$.
Therefore, the leader can prove that the predicate $D_j$ has been signed by $q_j\lfloor \frac{t}{\tau} \rfloor$ processes, for every $j \in [1, J]$; note that $q_j\lfloor \frac{t}{\tau} \rfloor \geq z_j - \lfloor \frac{t}{\tau} \rfloor + 1$.
Let $Z = \sum\limits_{j \in [1, J]} z_j$; observe that $Z \geq n - f \geq n - t$.
% Since $\forall j \in [1, J],  \exists q_j \in [0:\tau]$ such that $z_j \in [\frac{q_j \cdot t}{\tau}: \frac{(q_j + 1) \cdot t}{\tau} - 1]$, the leader can prove that the predicate $D_j$ has been signed by $\frac{q_j \cdot t}{\tau}$ processes, for every $j \in [j, J]$; note that $\frac{q_j \cdot t}{\tau} \geq z_j - \frac{t}{\tau} + 1$.
% Let $Z = \sum\limits_{j \in [1, J]} z_j$.
% $\forall j \in J$,
% the leader can prove the predicate $D_j$ has been signed by $\frac{q_j \cdot t}{\tau}$ processes (via threshold signature $TS^{\frac{q_j \cdot t}{\tau}}(P_j)$) that is by at least $z_j - \frac{t}{\tau} + 1$. We note $Z = \sum_{j \in J} z_j$

Furthermore, the leader collects $S > Z - J \cdot \frac{t}{\tau}$ ``useful'' signatures (as $\frac{t}{\tau} \geq \lfloor \frac{t}{\tau} \rfloor$) which can be merged into no more than $\mathsf{max}(J)$ threshold signatures.
Since $Z \geq n-f$, it follows that $S > n-f -  J \cdot \frac{t}{\tau}$.
Therefore, $S > (2t+1) + (c - \frac{J}{\tau})t - f$.
Let $\tau = \lceil \mathsf{max}(J) \cdot \frac{2}{c} \rceil$. 
Finally, $S > (2t+1) + \frac{ct}{2} - f$.

At this point, there are two possible scenarios:
\begin{compactenum}
    \item $f \leq \frac{ct}{2}$: In this case, $S \geq (2t + 1)$ and we can prove that at least two correct processes have proposed different values.
    
    \item Otherwise, $f = \Theta(n)$. 
    In this case, we can use a quadratic fallback, which means that the ``adaptiveness'' of the certification phase is preserved.
\end{compactenum}

Lastly, we note that no fallback is required if $n = 4t + 1$ and $\tau \geq \mathsf{max}(J)$ as, in this case, $S \geq 3t + 1 - J\frac{t}{\tau}$.
Hence, we need to have that $J\frac{t}{\tau} \leq t$, which implies that $\tau \geq J$.
Since $\mathsf{max}(J) = 7$ (by \Cref{lemma:upper_bound_size_of_partition}), $\tau \geq 7$ guarantees that, in the case of $n = 4t + 1$, no fallback is required.
% \jovan{It is important here that the leader cannot immediately go to the fallback as correct processes cannot then distinguish this scenario from a case in which the leader is Byzantine and forces the fallback immediately (even though the leader is the only Byzantine process). We must wait $\frac{ct}{2}$ rounds before going to the fallback. Am I missing something?}
% \pierre{Well, in the algorithm \ref{algorithm:consensus}, the fallback is not triggered by a leader, it is triggered after $\frac{c}{2}t +1$ phases, if either (i) $t+1$ \textsc{help-req} messages or (ii) a $(t+1)$ \textsc{fall-back} quorum-certificate made of $t+1$ \textsc{help-req} messages are received (and then forward) by a correct process. This can happen only if $f > \frac{c}{2}t$.}

\smallskip
\noindent \textbf{Intermediate results.}
We now present a few intermediate results.

\begin{lemma}\label{lemma:lower_bound_multiplicity_of_sub_partition}
Let $(G_{j})_{j \in [1, J]}$ be a partition of a set of values  such that (1) $J \geq 2$, and (2) $\forall j,j' \in [1, J], \#(G_j)+\#(G_{j'}) \geq t+1$.
Then, for every $k \geq 2$ and every sequence $j_1, ..., j_k \in [1, J]$,
$\#(G_{j_1})+\#(G_{j_2})+...+\#(G_{j_k}) \geq k \frac{(t+1)}{2}$.
\end{lemma}

\begin{proof}
Without loss of generality, let $\#(G_1) \leq ... \leq \#(G_{J})$.
Since $\#(G_1) \leq \#(G_2)$ and $\#(G_1) + \#(G_2) \leq t + 1$, we have that $\#(G_2) \leq \frac{t + 1}{2}$.
Therefore, for every $j > 1$, $\#(G_j) \geq \frac{t + 1}{2}$.

Finally, $\#(G_{j_1})+\#(G_{j_2})+...+\#(G_{j_k}) = \big(\#(G_{j_1}) + \#(G_{j_2})\big) + \#(G_{j_3}) + ... + \#(G_{j_k}) \geq (t + 1) + (k - 2)\frac{t + 1}{2} = 2\frac{t + 1}{2} + (k - 2)\frac{t + 1}{2} = \frac{t + 1}{2}(2 + k - 2) = k\frac{t + 1}{2}$.
Hence, the lemma holds.
\end{proof}

\begin{lemma}\label{lemma:lower_bound_size_of_partition}
Let $(G_{j})_{j \in [1, J]}$ be a partition of a set of values $V$ with $\#(V) \geq 2t+1$ such that $\forall j \in [1, J], \#(G_j) \leq t$.
Then, $J \geq 3$.
\end{lemma}
\begin{proof}
We assume that, by contradiction, $J \leq 2$.
Then, $\#(V) \leq 2t$, which contradicts the fact that $\#(V) \geq 2t + 1$.
Thus, the lemma holds.
\end{proof}

\begin{lemma}\label{lemma:upper_bound_size_of_partition}
Let $(G_{j})_{j \in [1, J]}$ be a partition of a set of values $V$ with $\#(V) \leq n = at+1$ such that (1) $a \geq 2$, (2) $\forall j,j' \in [1, J], \#(G_j)+\#(G_{j'}) \geq t+1$, and (3) $\forall j \in [1, J], \#(G_j) \leq t$.
Then, $J \leq \lceil 2a \rceil -1$.
\end{lemma}

\begin{proof}
Without loss of generality, let $\#(V) = n = at + 1$.
By \Cref{lemma:lower_bound_size_of_partition}, we have $J \geq 3$.
By \Cref{lemma:lower_bound_multiplicity_of_sub_partition}, we have that $\#(V) \geq \frac{J}{2}(t + 1)$.

By contradiction, let $J \geq \lceil 2a \rceil$.
Hence, $\#(V) \geq \frac{\lceil 2a \rceil}{2}(t + 1) \geq a(t + 1)$.
For every $a \geq 2$, we have that $a(t + 1) > at + 1$, which contradicts $\#(V) = n$.
Therefore, the lemma holds.
\end{proof}

\begin{lemma}\label{lemma:precision}
Let the leader receive $z_j \leq t$ well-formed \textsc{confirm} messages with $\tau$ partial signatures for group $G_j$: $\mathit{PS}^{\lfloor \frac{t}{\tau} \rfloor}, \mathit{PS}^{2\lfloor \frac{t}{\tau} \rfloor}, ..., \mathit{PS}^{\tau \lfloor \frac{t}{\tau} \rfloor}$. 
Then, the leader can compute a $(s_j,n)$-threshold signature for group $G_j$  with $z_j - s_j \leq  \lfloor \frac{t}{\tau} \rfloor - 1$.
%with $s_j \geq z_j - \lfloor \frac{t}{\tau} \rfloor + 1$.
\end{lemma}

\begin{proof}
The Euclidian division of $z_j$ by $\frac{t}{\tau}$ gives
$z_j = x_z \lfloor \frac{t}{\tau} \rfloor + y_z $ with $y_z \in [0, \lfloor \frac{t}{\tau} \rfloor-1]$ and $x_z \in [0, \tau]$.
Hence, the leader can combine $x_z \lfloor \frac{t}{\tau} \rfloor$ $(x_z \lfloor \frac{t}{\tau} \rfloor,n)$-partial signatures to obtain an $(x_z\lfloor \frac{t}{\tau} \rfloor,n)$-threshold signature. Finally, $z_j - x_z \lfloor \frac{t}{\tau} \rfloor = y_z \leq \lfloor \frac{t}{\tau} \rfloor-1$, which concludes the proof.

\end{proof}

\subsection{More Sophisticated Analysis: $\tau$ is Independent of $c$}

The previous analysis is conservative. 
The goal of a certificate $\Psi_{w}$ attached to the value $w$ is to ensure that deciding $w$ cannot violate the strong validity property, i.e., either (C1) a correct process proposed $w$, or (C2) at least two correct processes proposed two different values. 

Let the leader propose a value $w$ with a certificate $\Psi_{w} = (\mathit{TS}_1, ..., \mathit{TS}_{|J|})$ , where (1) $|J|\geq 3$, (2) $\sum\limits_{j \in J} \mathit{TS}_j \geq t + 1$, and (3) $\forall j \in J$, $\mathit{TS}_{j}$ is an $(s_j, n)$ threshold signature for a group $G_j$. 
Thus, it is sufficient for the leader to ensure that (C1') there exists $j^* \in J$ such that $\mathit{TS}_{j^*}$ is an $(t + 1, n)$ digital signature of $w$, or (C2') for every $j^* \in J$, $\sum\limits_{j \in J \setminus{\{j^*\}}} (|TS_j|) \geq t + 1$.
Note that C1' implies C1.
Moreover, note that C2' implies C2 as, once we ``remove'' $t$ potentially faulty processes, we are left with $t + 1$ processes which must ``belong'' to (at least) two different groups (as each group can have at most $t$ processes; see the second constraint on the group construction).

In the rest of this section, we deal with two scenarios: (1) $|J| \geq 4$, and (2) $|J| = 3$ (recall that $|J| \geq 3$ by \Cref{lemma:lower_bound_size_of_partition}).

\smallskip
\noindent \textbf{First case: $|J| \geq 4$.}
Firstly, recall that, for every $j, j' \in J$, $\#(G_j) + \#(G_{j'}) > t$.
Hence, at most one group can ``completely'' be Byzantine.
Therefore, we are left with (at least) three groups that contain a correct process. Thus the idea is to provide a certificate with $|J|$ threshold-signatures, whose thresholds $(s_j)_{j \in J}$ verify: $\forall j^* \in J$, $\sum\limits_{j \in J \setminus{\{j^*\}}} s_j \geq t+1$. Hence, there is no way that the provider of such a certificate, "hide" a value $v_{j^*}$ (in a multiset $G_{j^*}$ for some $j^* \in J$)  that would be the unique value proposed by correct processes.  

Let $j^* \in J$.
Then, $\sum\limits_{j \in J \setminus{\{j^*\}}} (z_j) \geq 3\frac{t + 1}{2} - 3\lfloor \frac{t}{\tau} \rfloor + 3$ (by \Cref{lemma:lower_bound_multiplicity_of_sub_partition}).
Furthermore, $\sum\limits_{j \in J \setminus{\{j^*\}}} (z_j) > 3\frac{t + 1}{2} - 3\frac{t}{\tau} > 3\frac{t + 1}{2} - 3\frac{t + 1}{\tau}$.
Finally, we need to ensure that $3\frac{t + 1}{2} - 3\frac{t + 1}{\tau} \geq t + 1$, which is ensured for $\tau \geq 6$.
Hence, if $|J| \geq 4$, it suffices for $\tau$ to be equal to $6$ to satisfy C2'.

\smallskip
\noindent \textbf{Second case: $|J| = 3$.}


This case might appear more difficult, because a naive application of lemma \ref{lemma:lower_bound_multiplicity_of_sub_partition} and lemma \ref{lemma:precision} would only guarantee $\forall j^{*} \in J, \sum_{j \in J \setminus \{ j^{*}\}} s_j \geq \frac{2(t+1)}{2} - \lfloor \frac{t}{\tau} \rfloor + 2$ and so $\tau = O(1)$ would not be enough to guarantee $\sum_{j \in J \setminus \{ j^{*}\}} s_j \geq t+1$. We need to be less conservative. They are two key elements to remark. First, (*) if $G_3 = \{w\}$, the leader does not have to ensure (C2') but either (C2') or (C1').
Second (**), when $|J| = 3$ and $\#(V) \geq 2t+1$, it is impossible for the adversary to allocate approximately $\frac{t+1}{2}$ values only to each set $G_j$. 

\begin{itemize}
    \item Case well-balanced: $\forall j,j' \in J$ $|\#(G_j) - \#(G_{j}')| \leq q \cdot t$ i.e. $\#(G_1) \geq \frac{\#(V)}{3} - q \cdot t$. This case is symptomatic of remark (**). 
    
    Indeed, since we assumed $f \leq ct$, $\#(V) \geq 2t+1$, and we have $\forall j^{*} \in J$, $\sum_{j \in J \setminus \{ j^{*}\}} z_j \geq 2\frac{2t+1}{3} - q \cdot t$. By lemma \ref{lemma:precision},
    $\sum_{j \in J \setminus \{ j^{*}\}} s_j \geq 2\frac{2t+1}{3} - q \cdot t - 2\lfloor \frac{t}{\tau} \rfloor > t + \frac{t}{3} - q \cdot t - 2\lfloor \frac{t}{\tau} \rfloor$
 .In that case, $\frac{6}{\tau}  \leq   1 - 3q$ is enough to ensure (C2'). Typically, for $q = \frac{1}{6}$, $\tau = 12$ is enough.

\item Case not well-balanced with $G_3 = \{ w \}$. In that case, this is even better for the leader because it can also satisfy (C1'). Indeed, $j^{*} = 3$, so $\sum_{j \in J \setminus \{ j^{*}\}} z_j \geq (t+1) + q \cdot t$. By lemma \ref{lemma:precision}, $\sum_{j \in J \setminus \{ j^{*}\}} s_j \geq (t+1) + q \cdot t - 2\lfloor \frac{t}{\tau} \rfloor+2$. So $\tau \geq \frac{2}{q} $, i.e. $\tau = 12 $ is enough to ensure (C2'). 

\item Case not well-balanced with $G_3 = \{ w_1, ..., w_{M} \}$ with $|G_3|=M$ and $\#(w_1) \leq ... \leq  \#(w_{M})$. This is the only challenging case. To solve it, we will approximate the two previous cases with a new partition. We partition $G_3$ into $G'_{3}$ and $G''_{3} = \{w_{M}\}$. We note $m = \#(w_{M})$ the multiplicity of $w_{M}$ in $G_3$. There are two new cases to deal with, either $m$ is big or $m$ is low.

\begin{itemize}
    \item If $m$ is big (TO FORMALISE, $m\geq \frac{t}{6}$ should be fine) , the leader will suggest to decide $w=w_{M}$ and ask the replicas to sign a confirmation to groups $G1,G_2, G'_{3}, G''_{3}$ .
In that case $\forall j^{*} \in J$ with $G_{j^{*}} \neq G''$, $\sum_{j \in J \setminus \{ j^{*}\}} s_j \geq t+1+\frac{t}{6} - 3\frac{t}{\tau}$. Here, $\tau \geq 18$ is enough.

\item If $m$ is low (TO FORMALISE, $m\leq \frac{t}{6}$ should be fine), we will perform a new partition $G_3 = G_{31} \cup G_{32}$ with $|\#(G_{32}) - \#(G_{31})| \geq m$ and ask the replicas to sign a confirmation to groups $G1,G_2, G_{31}, G_{32}$. 
Then, $\forall j^{*} \in J$, $\sum_{j \in J \setminus \{ j^{*}\}} s_j \geq (t+1) + \frac{t}{2} - 2m  - 3\frac{t}{\tau} > \frac{3t}{2} - 2m - 3\frac{t}{\tau}$. So the leader just need $\frac{3t}{\tau} \leq \frac{t}{2} - 2m$. 
For $m = \frac{t}{6}$, $\frac{18t}{6\tau} \leq \frac{t}{6}$, i.e. $\tau \geq 18$ is enough. 
\end{itemize}

\end{itemize}

\paragraph*{Even better}

We can do certainly better with more subcases: typically $m$ big means $m \geq \frac{t}{3}$, $m$ low means $m \leq \frac{t}{12}$ and two new cases for $m \in [\frac{t}{12}: \frac{t}{6}]$ and $m \in [\frac{t}{6}: \frac{t}{3}]$ where $G_3$ is partitioned into $(G_{31}, G_{32}, G_{33} = \{w\})$

Subcase $m \in [\frac{t}{12}: \frac{t}{6}]$: 

$\forall j^{*} \in J$ with $G_{j^{*}} \neq G_{33}$, $\sum_{j \in J \setminus \{ j^{*}\}} s_j \geq t+1+\frac{4t}{12}+ \frac{t}{12} - 4\frac{t}{\tau}$ so $\frac{t}{\tau} \geq \frac{5t}{48}$ is enough i.e. $\tau \geq 10$ is enough.

Subcase $m \in [\frac{t}{6}: \frac{t}{3}]$: 

TO DO

\iffalse
\paragraph*{The big constants}
Some big constants appears here when $c \leq 0.5$. Indeed, in that case, the number $\tau$ of threshold signature schemes is equal to $\frac{10}{c}$ (resp. $\frac{6}{c}$ with the optimization), while the fallback appears with $\frac{c}{2}t$ failures only.
For $c = 0.5$, $\tau = 20$ (resp. $\tau = 12$ with the optimization) and the fallback occurs with $f = \frac{n}{10}+1$ only.
For $c = 0.1$, $\tau = 100$ (resp. $\tau = 60$ with the optimization) and the fallback occurs with $f = \frac{n}{42}+1$ only.

This analysis is quite conservative and some optimization can be found. Typically, if the leader collect 3 $(\frac{t}{2}, n)$ threshold signatures for as many pairwise disjoint sets of values + one unique partial-signature for one value, ($S=\frac{3t}{2}+1 <2t+1$), then this is still a valid certificate, since removing $t$ potentially Byzantine processes, always lead to at least two different values signed by two different correct processes. We can show (TO DO formally), that the worst case is by far, having $|J| = 3$ and $\#(G_1) = t$. This allow to use $\tau = \frac{6}{c}$ instead of $\tau = \frac{10}{c}$.

In practice, the cryptographic number $\kappa$ should be $256$. If $c$ is low and $n$ is not big (e.g. $c = 0.1$, $n \simeq 100$), an aggretated signature with $\kappa + n$ bits size will be more interesting. We can also use a compressed-signature with $O(\kappa\cdot log(n))$ bits if $n \simeq 5000$.

A dichotomy-based exchange can also allow a $O(\kappa \cdot log(\tau) \cdot f \cdot n)$ communication complexity instead of $O(\kappa \cdot \tau \cdot f \cdot n)$ if we accept a $O(f \cdot log(\tau))$ worst-case latency complexity.
After its partitioning, for every $j \in J$ the leader notes $z^{0}_j$ the cardinal of $G_j$.Then, he will interact with the nodes by asking them they confirm they indeed proposed a value in $G_j$ with a $(k_j^s,n)$ threshold-signature where $k_j^s$ will change in a dichotomy fashion at each step $s$.
At each step $s \geq1 $, the leader receives $z^{s}_j \leq z^{s-1}_j$ confirmations and $k_j^{s} = max \{q_j^s \cdot \frac{t}{\tau} | q_j^s \in [1;\tau] \wedge q_j^s \cdot \frac{t}{\tau} \leq (k_j^{s-1}+z^{s-1}_j)/2 \}$. At step $s = log_2(\tau)$, $k_j^{s+1} = k_j^{s}$.
\fi

==> sections/certification_problem.tex <==
\section{Certification: Problem Definition} \label{section:certification_problem_definition}

Certification is defined as a problem of obtaining a locally-verifiable, constant-sized cryptographic proof, which we call \emph{certificate}, that some value is valid according to some criterion.
We formally define the problem below.

Let $\mathsf{Value}$ denote the set of values.
Moreover, let $\mathsf{Certificate}$ denote the set of certificates.
A function $\mathsf{verify}$: $\mathsf{Value} \times \mathsf{Certificate} \to \{\mathit{true}, \mathit{false}\}$ is defined.
Intuitively, if $\mathsf{verify}(v, \Sigma) = \mathit{true}$, for some value $v \in \mathsf{Value}$ and some certificate $\Sigma \in \mathsf{Certificate}$, then $\Sigma$ proves that $v$ is a valid value.
Finally, the certification problem is associated with two parameters:
\begin{compactenum}
    \item Leader: A unique, predetermined \emph{leader} process.
    
    \item Optimistic threshold: A number of faults the problem tolerates while \emph{guaranteeing} an attainment of a certificate (see the liveness property of the problem).
\end{compactenum}
We underline that the upper bound on number of faults is $t$ (and not the optimistic threshold), as introduced in \Cref{section:model}.
The leader and the optimistic threshold are merely parameters of the problem specification.
If the leader is $L$ and the optimistic threshold is denoted by $t_{\mathit{opt}}$, we denote the specific certification problem as $(L, t_{\mathit{opt}})$-certification.

The $(L, t_{\mathit{opt}})$-certification problem exposes the following interface:
\begin{compactitem}
    \item \textbf{request} $\mathsf{start}(v \in \mathsf{Value})$: a process starts certification with a value $v$.
    
    \item \textbf{indication} $\mathsf{obtain\_certificate}(v' \in \mathsf{Value}, \Sigma' \in \mathsf{Certificate})$: a process obtains a certificate $\Sigma'$ for a value $v'$.
    
    \item \textbf{indication} $\mathsf{stop}$: a process stops certification.
\end{compactitem}

$(L, t_{\mathit{opt}})$-certification requires the following properties to be satisfied:
\begin{compactitem}
    \item \emph{Termination:} \pierre{If all the correct processes start at the same round ?} Every correct process eventually stops certification \pierre{at the same round ?}.

    \item \emph{Liveness:} If $L$ is correct and $f \leq t_{\mathit{opt}}$, every correct process eventually obtains a certificate $\Sigma'$ for some value $v'$ such that $\mathsf{verify}(v', \Sigma') = \mathit{true}$.
    
    \item \emph{Safety:} If all correct processes start certification with the same value $v$ and a (correct or faulty) process obtains a certificate $\Sigma'$ for a value $v'$, then $v = v'$. \footnote{A faulty process obtains a certificate $\Sigma$ if it stores $\Sigma$ in its local memory.}
\end{compactitem}
The termination property states that all correct processes eventually terminate certification.
Liveness guarantees that, if the leader is correct and the number of faults does not exceed the optimistic threshold, all correct processes eventually obtain a certificate for some value.
Finally, safety ensures that, if all processes start with the same value, no process (even if faulty) can obtain a certificate for any other value.

==> sections/consensus.tex <==
\section{From certification phase to consensus}

We transform the adaptive consensus with weak unanimity from \cite{Cohen2022} with our certification protocol of section \ref{section:certification} to obtain an adaptive consensus with strong unanimity. 

The algorithm follows a succession of leader-based phases (protocol \ref{algorithm:invocation_phase} and \ref{algorithm:invocation_phase_remaining}) with a different leader at each phase. 
At each phase, if enough processes are correct and none of them already decided,  a leader can make all the correct process agree on a valid value. To avoid that two different Byzantine leader make processes disagree, a quorum certificate of size $\lceil \frac{n + t + 1}{2} \rceil$ for value $v$ has to be obtained to decide $v$. Indeed, two quorum certificates of size $\lceil \frac{n + t + 1}{2} \rceil$ for value $v$ and $v'$ have necessarily been signed by $2(\lceil \frac{n + t + 1}{2} \rceil) - n \geq t+1$ different processes, and so by at least one correct process. If the algorithm is designed such that a correct process cannot partially-sign two different values, safety is ensured. The validity is ensured with the  certification's mechanism of previous section \ref{section:certification}. Now we explain how to ensure liveness.

They are two scenarios:
\begin{itemize}
    \item optimistic scenario: $f \leq \frac{c}{2}t \leq n -(\lceil \frac{n + t + 1}{2} \rceil)$:
    
    
    (1) the first correct leader will be able to produce both (i) a constant-sized proof of validity for some value $v$ for any input configuration and (ii) a quorum-certificate for value $v$ with threshold $\lceil \frac{n + t + 1}{2} \rceil \leq n- \frac{c}{2} t$.
When a process decide a value at phase $\phi$, and become leader at phase $\phi'>\phi$, he is mute by default, and only answers to requests from processes that pretend they did not answer yet. Upon such a request, he answers with its quorum-certificate. Hence, in optimistic scenario, all correct processes decide at phase $f+1$ \footnote{It seems this minor modification had been forgotten in \cite{Cohen2022}, which led to a non-adaptive $O(t)$ latency complexity. However, the fix is quite straightforward. }.  Moreover, the number of answers to false requests is bounded by $(t+1)\cdot f$. This lead to $O(f \cdot n)$ communication complexity in the worst case.
    
    
    \item pessimistic scenario: $f> \frac{c}{2} t$:
    In that case, $f = \Theta(n)$. So if consensus is not achieved, the processes fallback into the quadratic algorithm from Momose and Ren \cite{Momose2021} which leads again to $O(f \cdot n)$ communication complexity in the worst case.
    The fallback has to be triggered only if $f > \frac{c}{2}t$. After the sequence of leader-based phases. The processes that did not decide broadcast a \textsc{help-req} message to warn they did not decide and expect an answer. Upon the reception of such a \textsc{help-req} message, a correct process that already decided can answer with a \textsc{help} message that holds the decided value and the attached quorum certificate. No fallback is triggered if no correct process receives $t+1$ \textsc{help-req} message, which never happens if $f \leq \frac{c}{2}t$. 
    If one correct process decided, he will answer to all \textsc{help-req} messages. If no correct process decided, every correct process will receives $n-t$ \textsc{help-req} messages. A correct process $P_i$ that receives $n-t$ \textsc{help-req} messages can create a quorum-certificate $QC_{fallback}$ that will be disseminate to convince every correct process to participate to the fallback optimal (but non-adaptive) consensus algorithm. 
\end{itemize}

\subsection{The sequence of leader-based phases}

In line \ref{line:cons_seq_phases} of algorithm  \ref{algorithm:consensus}, the processes start a sequence of $\frac{c}{2}t+1$ leader-based phases. The leader is replaced at each new phase in a round-robin fashion. A phase $\phi$ is running as follows: At first round, if the leader already decided, he stays mute. Otherwise, he broadcast a \textsc{not-decided} message to inform very process that it needs their proposals to make a suggestion (This round can be obviously removed at first phase). At round $2$, if a process $P_i$ did not receive a \textsc{not-decided} message, but did not decide, he sends a \textsc{help-not-decided} message to the leader to request the decision (with a proof). Indeed, it might be possible that the current leader decided in a previous phase with a Byzantine leader that did not allow every correct process to decide. If the process $P_i$ did not receive an answer to its request at round $3$, he will now for sure that the current leader is not correct. At round $2$, if a process $P_i$ did not receive a \textsc{not-decided} message, and did decide as well, it does not do anything during the phase. Hence, if a correct process $P_i$ decides at phase $\phi$ and is leader at phase $\phi' \geq \phi$, (1) every correct process decides by phase $\phi'$, (2) there is no communication between two correct processes after phase $\phi'$, (3) $P_i$ can halt after phase $\phi'$. 

Let us go back to the round $2$ where process $P_i$ did receive a \textsc{not-decided} message. In that case it answer to the leader by sending him a \textsc{disclose} message containing its proposal, share-signed with a key of a $(t+1, n)$-threshold signature.

At round $3$, the leader that did not decide, receives between $n-f$ and $n$ \textsc{disclose} messages. If he receives less than $n-\frac{c}{2}t$ values, he stops to participate to the phase.

Otherwise, it checks if a value $v^*$ has been proposed $t+1$ times. If this is the case, it combine the attached share-signature to obtain $TS^{t+1}(v^*)$, a $(t+1, n)$-threshold signature of $v^{*}$. This is the proof that it is safe to decide $v^{*}$. Finally, he broadcasts a \textsc{unanimity} message containing $v^{*}$ and $TS^{t+1}(v^*)$, which means he suggests to decide $v^{*}$.

However, it is possible that no value is represented $t+1$ times. In that case,  he  partitions the received values into $|J|$ multisets $(G_j)_{j \in J}$ where $\forall j \in J$, $\#(G_j) \in [\frac{t}{2}:t]$. Then, for each $j \in J$ it multicasts a \textsc{partition} message with the description $D_j$ of set $G_j$ to each process that proposed a value in $G_j$. 

In round $4$, a process $P_i$ that received a \textsc{unanimity} message, store the attached threshold-signature $TS^{t+1}(v^*)$ and wait for round $6$.
a process $P_i$ that received a \textsc{partition} message for set $G$, with description $D$, that matches its proposal $v_i$ ($v_i \in G$), will send a \textsc{confirm} message to confirm he indeed sent a proposal $v_i$ in the set $G$. Moreover he attaches a sequence of $\tau$ threshold-signature of the description $D$ of $G$.

In round $5$, the leader that multicasted \textsc{partition} messages , receives between $n-f$ and $n$ \textsc{confirm} messages. If he receives less than $n-\frac{c}{2}t$ values, he stops to participate to the phase.
Otherwise, for each index $j \in J$, he select the $z_j$ \textsc{confirm} messages sent for group $G_j$. Among the $\tau$ threshold, he pick up the highest threshold $k_j$ which stays lower or equal than $z_j$. Then, he combines $k_j$ share-signatures of description $D_j$ of group $G_j$ to obtain a $(k_j,n)$-threshold signature $TS^{k_j}(D_j)$ of description $D_j$ of group $G_j$. 
Thereupon, he creates a certificate $\Psi_{ANY}$ by concatenating the pairs ($D_j, TS^{k_j}(D_j)$) for all the $j \in J$. Since $\sum_{j \in J}k_j \geq 2t+1$, it constitutes a proof that it is impossible that all the correct processes proposed the same value.
Finally, he broadcast a \textsc{allow-any} message with the proof $\Psi_{ANY}$ and its own proposal $v_{leader}$ that can be decided safely.

A process that received value $w$ via either a \textsc{unanimity} message in round $4$ with the proof $\Psi_{w}$ or a \textsc{allow-any} message in round $6$ with the proof $\Psi_{ANY}$ knows the leader suggests to decide value $w$.
However, we have to ensure agreement for every number $f \leq t$ of Byzantine failures. This is the role of the quorum-certificates of size $\lceil \frac{n+t+1}{2} \rceil$.

Thus, in round 6, if process $P_i$ did not commit another value, he sends a \textsc{vote} message with $(\lceil \frac{n+t+1}{2} \rceil, n)$ share signature $(\textsc{vote},
w)$. If $P_i$ already commited another value $v^c$, he sends a \textsc{commit} message with $v^c$ and the attached quorum-certificates $QC_{commit}(v^c_i)$ of size $\lceil \frac{n+t+1}{2} \rceil$. 
In round $7$, if the leader received a \textsc{commit} message, it changes it suggestion and forward the  \textsc{commit} message to everyone. Otherwise, it received only \textsc{vote} messages. If it received less than  $\lceil \frac{n+t+1}{2} \rceil$ \textsc{vote} messages, it stops to participate to this phase. If it received  $\lceil \frac{n+t+1}{2} \rceil$ \textsc{vote} messages, it combine the threshold signatures to create a quorum certificate $QC_{commit}(w)$ that it broadcast in a \textsc{commit} message.

In round $8$, a process $P_i$ that received a \textsc{commit} message for value $v^c$, store the attached quorum-certificate $QC_{commit}(v^c) = TS^{\lceil \frac{n+t+1}{2} \rceil}(\textsc{vote}, v^c, \phi' \leq \phi)$ and send a \textsc{decide} message for value $v^c$ to the leader with $(\lceil \frac{n+t+1}{2} \rceil, n)$ share signature for $(\textsc{decide},
v^c)$. 

In round $9$, if the leader received less than  $\lceil \frac{n+t+1}{2} \rceil$ \textsc{decide} messages, it stops to participate to this phase. If it received  $\lceil \frac{n+t+1}{2} \rceil$ \textsc{decide} messages, it combine the threshold signatures to create a quorum certificate $QC_{finalize}(v^c)$ that it broadcast in a \textsc{finalize} message.

In round $10$, a process $P_i$ that received a \textsc{finalize} message for value $v^c$, store the attached quorum-certificate $QC_{finalize}(v^c) = TS^{\lceil \frac{n+t+1}{2} \rceil}(\textsc{decide}, v^c, \phi)$ and decides $v^c$.



\begin{algorithm} [ht]
\caption{$\mathsf{invocation Phase}(leader, v_i)$: Pseudocode for process $P_i$}
\label{algorithm:invocation_phase}
\begin{algorithmic} [1]

\State \textbf{constant }
%\State $leader \gets \ell$
 \State $\tau = \frac{4(2+c)}{c} = 4 + \frac{8}{c}$; $\forall q \in [1:\tau], k_q = q\frac{t}{\tau}$ 
\State \textbf{Round 1:}  \BlueComment{propose value $\mathit{proposal}$}
\State \textbf{if } $P_i = leader$ $\wedge$ $decided = \bot$:
\State \hskip2em \textbf{broadcast } $\langle \textsc{not-decided} \rangle_{leader}$

\State \textbf{Round 2:}
\State \textbf{if } $\langle \textsc{not-decided} \rangle_{leader}$ received:
\State \hskip2em \textbf{send} $\langle \textsc{disclose}, v_i, \mathit{ShareSign}^{t+1}_i(v_i) \rangle$ to leader 
\BlueComment{informing the leader of his proposal} \label{line:send_disclose} 
\State \textbf{else }:
\State \hskip2em \textbf{if } $decided = \bot$: 
\State \hskip4em \textbf{broadcast } $\langle \textsc{help-not-decided} \rangle_{P_i}$ to leader

\smallskip
\State \textbf{Round 3} (if $P_i = leader$) \textbf{:} 
\State \textbf{if} $decided \neq \bot$:
\State \hskip2em for every $P_j$ whose message $\langle \textsc{help-not-decided} \rangle_{P_j}$ has been received, \textbf{send} $\langle \textsc{rescue}, decided, decideProof, validityProof  \rangle$

\State \textbf{else:} 
\State \hskip2em \textbf{if} exists $\mathsf{Value}$  $v$ such that $\langle \textsc{disclose}, v, \mathsf{P\_Signature}  \mathit{sig}\rangle$ is received from $2t+1$ processes: 
\State \hskip2em \textcolor{blue}{\(\triangleright\) a certificate for $v$ is obtained}
\State \hskip4em $\mathsf{Certificate}$ $\;$ $\Psi_v \gets \mathit{Combine}(\{\mathit{sig} \,|\, \mathit{sig} \text{ is received in a } \textsc{disclose} \text{ message}\})$ 
\State \hskip4em \textbf{broadcast} $\langle \textsc{UNANIMITY}, v, \Psi_v \rangle$ \BlueComment{disseminate the certificate} 

\State \hskip2em \textbf{else:}
\State \hskip4em $(\underline{G}, \underline{D}, J) \gets \mathsf{Partition}(\{values | values \text{ received in } \textsc{DISCLOSE} \text{ messages }\})$
\State \hskip4em for every $j \in J$, for every process $P_q$ s.t. $v_q \in P_j$, \textbf{send}  $\langle \mathsf{PARTITION}, D_j   \rangle_{leader}$ to $P_q$

\smallskip
\State
\textbf{Round 4:}
\State \textbf{if} received $\langle \mathsf{uninamity}, v, \Psi_{v}  \rangle_{leader}$
\State \hskip2em $certificate_i \gets \Psi_v$ 
\State \hskip2em $proposal_i[leader] \gets v$ 
 \BlueComment{Wait for round 6}
%\State \hskip2em \textbf{return}
\State \textbf{if} received $\langle \mathsf{PARTITION}, D   \rangle_{leader}$ such that $\mathsf{Match}(v_i, D)$:
\State \hskip2em \textbf{send} $\langle \mathsf{CONFIRM}, D, [\mathit{ShareSign}^{k_1}_i(D), ..., \mathit{ShareSign}^{k_\tau}_i(D)] \rangle_{i}$ to $leader$

\smallskip
\State \textbf{Round 5} (if $P_i = leader$) \textbf{:} 
\State Let $ConfirmMessages$ the set of well-formed received \textsc{CONFIRM} messages

\State \textbf{if} $Card(ConfirmMessages)\geq$ $(2+\frac{c}{2})t+1$: 
\State \hskip2em $\Psi_{ANY} \gets \mathsf{BuildAllowAnyCertificate}(ConfirmMessages, \underline{D}, J)$


 \State \hskip2em \textbf{broadcast} $\langle \textsc{allow-any}, v_i, \Psi_{ANY} \rangle_{leader}$

\State \textbf{else:}
\State \hskip2em \textbf{return} \BlueComment{There is $\frac{c}{2}t = \Theta(t)$ failures, which allows a fallback to a quadratic protocol (like \cite{Momose2021})}

\State \BlueComment{To Follow...}

\end{algorithmic}
\end{algorithm}

\begin{algorithm} [ht]
\caption{Follow-up of $\mathsf{invocation Phase}(leader, v_i)$: Pseudocode for process $P_i$}
\label{algorithm:invocation_phase_remaining}
\begin{algorithmic} [1]

\State
\textbf{Round 6:}
\State \textbf{if} received $\langle \textsc{allow-any}, v, \Psi_{ANY} \rangle_{leader}$:
\State \hskip2em $certificate_i \gets \Psi_{ANY}$
\State \hskip2em $proposal_i[leader] \gets v$
\State \textbf{if} $proposal_i[leader] \neq \bot \wedge commit_i = \bot$:
\State \hskip2em \textbf{send} $\langle \textsc{vote}, proposal_i[leader] \rangle_{P_i}$ to leader
\State \textbf{else if} $proposal_i[leader] \neq \bot \wedge commit_i \neq \bot$:
\State \hskip2em \textbf{send} $\langle \textsc{commit}, commit_i, commitProof_i \rangle_{P_i}$ to leader

\smallskip
\State
\textbf{Round 7:}

\textbf{if} received $\langle \textsc{commit}, v,QC_{commit}(v), \rangle_{P_i}$: \State \hskip2em
\textbf{broadcast} the message $\langle \textsc{commit}, v,QC_{commit}(v), \rangle_{leader}$ 
\State
\textbf{else if} received $\lceil \frac{n+t+1}{2}\rceil$ messages of $\langle \textsc{vote}, v, \rangle_{P_j}$:
\State \hskip2em batch these messages into $QC_{commit}(v)$ using a $(\lceil \frac{n+t+1}{2}\rceil,n)$-threshold signature scheme
\State \hskip2em \textbf{broadcast} the message $\langle \textsc{commit}, v,QC_{commit}(v) \rangle_{leader}$


\smallskip
\State
\textbf{Round 8:}
if received $\langle \textsc{commit}, v,QC_{commit}(v) \rangle_{leader}$:
\State \hskip2em \textbf{send} $\langle \textsc{decide}, v \rangle_{P_i}$ to leader
\State \hskip2em \textbf{if} $commit_i= \bot$ then
$commit_i \gets v$
$commitProof_i \gets QC_{commit}(v)$

\smallskip
\State
\textbf{Round 9:}
\State \textbf{if} $leader = P_i$:
\State \hskip2em \textbf{if} received $\lceil \frac{n+t+1}{2}\rceil$ messages of $\langle \textsc{decide}, v, \rangle_{P_j}$: 
\State \hskip4em batch these messages into $QC_{finalized}(v)$ using a $(\lceil \frac{n+t+1}{2}\rceil,n)$-threshold signature scheme
\State \hskip4em \textbf{broadcast} the message $\langle \textsc{finalized}, v,QC_{finalized}(v) \rangle_{leader}$

\State \textbf{if} received $\langle \textsc{finalized}, v,QC_{finalized}(v) \rangle_{leader}$: 
\State \hskip2em $decided_i \gets v$ 
\State \hskip2em $decidedProof_i \gets QC_{finalized}(v)$

\State \textbf{return}$(decided_i,decidedProof_i,commit_i,commitProof_i)$
     
\end{algorithmic}
\end{algorithm}

\subsection{The adaptive consensus with potential fallback}

The adaptive consensus presented in algorithm \ref{algorithm:consensus} is quasi the same than the adaptive consensus of \cite{Cohen2022}. The first difference is that it calls a new invocation phase with a new certification phase to ensure strong validity. The second difference is that the fallback can be triggered with a small number $f > \frac{c}{2(2+c)}n$ of failures instead of $f> \frac{n}{4}$ in \cite{Cohen2022}.

If $f \leq \frac{c}{2}t$, all the correct processes decide by the phase $f+1$ led by the first correct leader. 
If $f \geq \frac{c}{2}t$, after the sequence of $\frac{c}{2}t+1$, it is possible that some correct processes did not decide.
The processes that did not decide broadcast a \textsc{help-req} message to warn they did not decide and expect an answer. Upon the reception of such a \textsc{help-req} message, a correct process that already decided can answer with a \textsc{help} message that holds the decided value $v$ and the attached quorum certificate $QC_{finalize}(v)$. No fallback is triggered if no correct process receives $t+1$ \textsc{help-req} message, which never happens if $f \leq \frac{c}{2}t$. 
    If one correct process decided, he will answer to all \textsc{help-req} messages. If no correct process decided, every correct process will receives $n-t \geq t+1$ \textsc{help-req} messages. A correct process $P_i$ that receives $t+1$ \textsc{help-req} messages can create a quorum-certificate $QC_{fallback}$ that will be disseminate to convince every correct process to participate to the fallback optimal (but non-adaptive) consensus algorithm.
    
    The last challenge is to synchronize the start of the fallback algorithm $\mathcal{A}_{fallback}$ (By default, $\mathcal{A}_{fallback}$ can be the Momose\&Ren's algorithm from \cite{Momose2021}). This is solved in Round $3$ of algorithm \ref{algorithm:consensus}, whose aim is to ensure that, in a window of $\delta$ time, all correct processes start $\mathcal{A}_{fallback}$ with a round time of $\delta' = 2 \delta$. A correct process $P_i$ starts $\mathcal{A}_{fallback}$ at time $fallbackStart_i$. As soon as possible, a correct process broadcast (or forward) a \textsc{fallback} message with attached quorum-certificate $QC_{fallback}$. The correct process schedules the start of $\mathcal{A}_{fallback}$,  $2\delta$ time after this moment. If possible, a \textsc{fallback} messages contain a proof $QC_{finalized}(v)$ of decision $v$ of the previous-phase. In that case, $v$ is adopted as proposal for $\mathcal{A}_{fallback}$. 
    If a correct process decided in the previous phase, $QC_{finalized}(v)$ will be obtain by all the correct processes before the start of $\mathcal{A}_{fallback}$ and 
     then all the correct processes will adopt $v$ as proposal. By strong validity, $v$ will be adopted, which ensures agreement between correct processes that decide in the previous phase and correct processes that decide in fallback.
     Also, if strong validity imposed that $v^{*}$ was the only possible value to decide, it is impossible for Byzantine processes to obtain $QC_{finalized}(v)$ for a non-valid value $v \neq v^{*}$, so correct processes will not change their proposal for the fallback, and by strong validity of the fallback algorithm, they will decide $v^{*}$. Hence, strong validity is preserved by the fallback mechanism.

%%%%%%%%%%%%%%%%
\begin{algorithm} [ht]
\caption{$\mathsf{consensus}( v_i)$: Pseudocode for process $P_i$}
\label{algorithm:consensus}
\begin{algorithmic} [1]

\State \textbf{Initially}
\State $fallBackStart_i \gets \infty$ 
  $decided_i, decidedProof_i, commit_i, commitProof_i,  fallbackVal_i, phaseDecision_i = \bot$
  
\State \textbf{for} $\ell \in [1:\frac{c}{2}t+1]$: \label{line:cons_seq_phases}

\State \hskip2em $phaseDecision_i,decideProof_i,commit_i,commitProof_i \gets invokePhase(\ell, v_i, commit_i, commitProof_i, decided_i)$ \State \hskip2em \textbf{if} $decided_i = \bot$ and $phaseDecision_i \neq \bot$ then
$decided_i \gets phaseDecision_i$

\State \textbf{Round 1:}
\State \textbf{if} $decided_i = \bot$:
\State \hskip2em
\textbf{broadcast} $\langle \textsc{help-req} \rangle_{P_i}$

\State \textbf{Round 2:}
\State \textbf{if}  received $\langle \textsc{help-req} \rangle_{P_j}$ message and $decided_i \neq \bot$:
\State \hskip2em
\textbf{send} $\langle\textsc{help},decided_i,decideProof_i \rangle_{P_i} $ to $P_j$.


\State \textbf{if} received $t+1$ messages of $\langle \textsc{help-req} \rangle_{P_j}$ from different processes:
\State \hskip2em batch these messages into $QC_{fallback}$ using a $(t+1,n)$-threshold signature scheme 
\State \hskip2em \textbf{broadcast} $\langle\textsc{fallback},QC_{fallback}, decided,decideProof \rangle_{P_i}$ 
\State \hskip2em $fallbackStart_i \gets now + 2\delta$

\State \textbf{Round 3:}
\State \textbf{if} received $\langle\textsc{help},v,QC_{finalized}(v) \rangle_{P_j} $ $\wedge$ $decided_i = \bot$:
\State \hskip2em $decided_i \gets v$ 

\State $updateDecision_i \gets v_i$ 
\State \textbf{if} $decided_i \neq \bot$:
\State \hskip2em $updateDecision_i \gets decided_i$ 

\State \textbf{while} $fallbackStart>now$: 
\State \hskip2em \textbf{if:} received valid $\langle\textsc{fallback},QC_{fallback}, v_j, decisionProof_j \rangle_{P_j}$:

\State \hskip4em \textbf{if:} $decided_i=\bot \wedge decisionProof_j \neq \bot$ 

\State \hskip6em $updateDecision_i \gets v_j$
\State \hskip6em $updateProof_i \gets decisionProof_j$

\State \hskip4em \textbf{if:} $fallbackStart = \infty$:
\State \hskip6em \textbf{broadcast}  $\langle\textsc{fallback},QC_{fallback}, updateDecision_i, updateProof_i \rangle_{P_i}$ \State \hskip6em $fallbackStart \gets now + 2\delta$

\State \textbf{return} $ \mathcal{A}_{fallback} $ with round duration of $\delta' = 2\delta$ and $updateDecision_i$ as proposal.


\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%
\iffalse
\begin{algorithm} [ht]
\caption{$\mathsf{invocation Phase}(leader, v_i)$: Pseudocode for process $P_i$}
\label{algorithm:invocation_phase}
\begin{algorithmic} [1]

%Sending Phase proposal
\State \textbf{constant }
%\State $leader \gets \ell$
 \State $\tau = \frac{4(2+c)}{c} = 4 + \frac{8}{c}$; $\forall q \in [1:\tau], k_q = q\frac{t}{\tau}$ 
\State \textbf{Round 1:}  \BlueComment{propose value $\mathit{proposal}$}
\State \textbf{if } $P_i = leader$ $\wedge$ $decided = \bot$:
\State \hskip2em \textbf{broadcast } $\langle \textsc{not-decided} \rangle_{leader}$

\State \textbf{Round 2:}
\State \textbf{if } $\langle \textsc{not-decided} \rangle_{leader}$ received:
 \label{line:certification_phase_start}
\State \hskip2em \textbf{send} $\langle \textsc{disclose}, v_i, \mathit{ShareSign}^{2t+1}_i(v_i) \rangle$ to leader \BlueComment{informing the leader of his proposal} \label{line:send_disclose} 
\State \textbf{else }:
\State \hskip2em \textbf{if } $decided = \bot$: 
\State \hskip4em \textbf{broadcast } $\langle \textsc{help-not-decided} \rangle_{P_i}$ to leader

\smallskip
\State \textbf{Round 3} (if $P_i = leader$) \textbf{:} 
\State \textbf{if} $decided \neq \bot$:
\State \hskip2em for every $P_j$ whose message $\langle \textsc{help-not-decided} \rangle_{P_j}$ has been received, \textbf{send} $\langle \textsc{rescue}, decided, decide\text{_}proof, validity\text{_}proof  \langle$

\State \textbf{else:} 
\State \hskip2em \textbf{if} exists $\mathsf{Value}$  $v$ such that $\langle \textsc{disclose}, v, \mathsf{P\_Signature}  \mathit{sig}\rangle$ is received from $2t+1$ processes: \label{line:2t+1_disclose}
\State \hskip2em \textcolor{blue}{\(\triangleright\) a certificate for $v$ is obtained}
\State \hskip2em $\mathsf{Certificate} \Psi_v \gets \mathit{Combine}(\{\mathit{sig} \,|\, \mathit{sig} \text{ is received in a } \textsc{disclose} \text{ message}\})$ \label{line:combine_certification_phase}
\State \hskip2em \textbf{broadcast} $\langle \textsc{certificate}, v, \sigma_v \rangle$ \BlueComment{disseminate the certificate} \label{line:broadcast_certificate_1}

\State \textbf{else:}
\State \hskip2em $(\underline{G}, \underline{D}, J) \gets \mathsf{Partition}(\{values | values \text{ received in } \textsc{DISCLOSE} \text{ messages }\})$
\State \hskip2em for every $j \in J$, for every process $P_q$ s.t. $v_q \in P_j$, \textbf{send}  $\langle \mathsf{PARTITION}, D_j   \rangle_{leader}$ to $P_q$

\smallskip
\State
\textbf{Round 3:}
\State \textbf{if} received $\langle \mathsf{CERTIFICATE}, v, \Psi_{v}  \rangle_{leader}$
\State \hskip2em $certificate_i \gets \Psi_v$ 
\State \hskip2em \textbf{return}
\State \textbf{if} received $\langle \mathsf{PARTITION}, D   \rangle_{leader}$ such that $\mathsf{Match}(v_i, D)$:
\State \hskip2em \textbf{send} $\langle \mathsf{CONFIRM}, D, [\mathit{ShareSign}^{k_1}_i(D), ..., \mathit{ShareSign}^{k_\tau}_i(D)] \rangle_{i}$ to $leader$

\smallskip
\State \textbf{Round 4} (if $P_i = leader$) \textbf{:} 
\State Let $ConfirmMessages$ the set of well-formed received \textsc{CONFIRM} messages

\State \textbf{if} $Card(ConfirmMessages)\geq$ $(2+\frac{c}{2})t+1$: 
\State \hskip2em $\Psi_{ANY} \gets \mathsf{BuildAllowAnyCertificate}(ConfirmMessages, \underline{D}, J)$


 \State \hskip2em \textbf{broadcast} $\langle \textsc{allow-any}, \Psi_{ANY} \rangle_{leader}$
 
 %\State \textbf{if} $Card(ConfirmMessages) \in $ $[2t+1: (2+\frac{c}{2})t+1($
%\State \hskip2em $\Psi_{ANY} \gets \{\text{received } \textsc{disclose} \text{ messages} \}$ \BlueComment{There is $\frac{c}{2}t = \Theta(t)$ failures, which allows a linear proof}
%\State \hskip2em \textbf{broadcast} $\langle \textsc{allow-any}, \Psi_{ANY} \rangle_{leader}$

\State \textbf{else:}
\State \hskip2em \textbf{return} \BlueComment{There is $\frac{c}{2}t = \Theta(t)$ failures, which allows a fallback to a quadratic protocol (like \cite{Momose2021})}


\smallskip
\State
\textbf{Round 5:}
\State \textbf{if} received$\langle \textsc{allow-any}, \Psi_{ANY} \rangle_{leader}$
\State \hskip2em $certificate_i \gets \Psi_{ANY}$
\State \hskip2em \textbf{return}
\end{algorithmic}
\end{algorithm}

\fi


==> sections/impossibility_results.tex <==
\section{Why should the case $n=(2+o(1))t+O(1)$ be impossible ?}
 The leader receives $ t-\alpha(t)$ times the value $0$ and $ t-\alpha(t)$ times the value $1$ with $\alpha(t) = o(t)$. 
The leader collect the signatures and produce a certificate (we do not care about the size of the certificate).

Now we have to deal with the two following scenarios:

Scenario $A_1$: the correct leader sends the collected signed proposals to justify both $0$ and $1$ can be decided. 

Scenario $B_1$: the Byzantine leader ignored $2\alpha(t)$ proposals for the same value $v^{*} \in \{0,1\}$, while all the processes that proposed $1-v^{*}$ are also faulty. 
The validity property requires that $v^{*}$ is the only value that can be decided.

This indistinguishability remains true with a sequence of $t$ leader based phases. 

We can extend this reasoning to show that each correct process has to receive at least $t+1$ messages, even in executions with only $o(t)$ failures.

\begin{definition}[Optimal Consensus]
An \emph{optimal consensus protocol} is a distributed protocol $\Pi$ that solves the synchronous Byzantine consensus with strong unanimity among $n$ processes with $t$-resiliency where $n=2t+1$. We note $Execs_{\Pi}(f)$ the set of executions of $\Pi$ with at most $f \leq t$ failures . We note $Execs_{\Pi}^{+}(f)$ the subset of $Execs_{\Pi}(f)$ where both liveness and safety is ensured. An execution $e$ is $J$-centralised, with $J \subseteq \Pi$, if each correct process interact with process in $J$ only.
\end{definition}

\begin{theorem}[leader-based protocol does not provide adaptiveness]
Let $\Pi$ be an \emph{optimal consensus protocol}. Let $\alpha : t \mapsto \mathbb{R}$ with $\omega(1) = \alpha(t) = o(t)$. Let $t, n \in \mathbb{N}$ s.t. $n=2t+1$. Then, there exists $e \in Execs_{\Pi}^{+}(\alpha(t)+1)$ that is not $J$-centralised with $|J| = \alpha(t)$. 
\end{theorem}

\begin{proof}
By contradiction, let us construct $e \in Execs_{\Pi}^{+}(\alpha(t)+1)$ which is $J$-centralised with $|J| = \alpha(t)$. 
We construct $\{G,H,J,R\}$ as a partition of $\Pi$ as follows:
\begin{itemize}
    \item $|G| = t-\alpha(t)$
    \item $G$ has $0$ as input
    \item $|H| = t-\alpha(t)$
    \item $H$ has $1$ as input
    \item $|R| = \alpha(t)+1$
    \item $R$ has $v^{*} \in \{0,1\}$ as input
    \item $|J| = \alpha(t)$
\end{itemize}

In execution $e$, processes in $R$ crash and a value $v_e \in \{0,1\}$ is decided by all the remaining correct processes. We have $\alpha(t)+1$ failures and potentially a message complexity of $O(n  \cdot |J|)$.

We construct $e_0$ where processes in $G \cup R$ are correct and processes in $H \cup J$ are Byzantine. The validity property implies $0$ has to be decided. 
The nodes in $J$ ignore $R$ and behave with the remaining nodes as in $e$. Hence $e_0$ is undistinguishable from $e$ for $G$.

We construct $e_1$ where processes in $H \cup R$ are correct and processes in $G \cup J$ are Byzantine. The validity property implies $1$ has to be decided. 
The nodes in $J$ ignore $R$ and behave with the remaining nodes as in $e$. Hence $e_1$ is undistinguishable from $e$ for $H$.

Thus, processes in $G$ have to decide $0$ in $e$, while processes in $H$ have to decide $1$ in $e$, which leads to disagreement and so a contradiction.

Conclusion, there exists $e \in Execs_{\Pi}^{+}(\alpha(t)+1)$ that is not $J$-centralised with $|J| = \alpha(t)$.

\end{proof}

==> sections/optimistic_case.tex <==
\section{\fast: \name's Fastest Path} \label{subsection:fast}

We start by presenting \fast, a straightforward fastest path of \name that ensures a decision in $2$ rounds with $2n$ exchanged bits in the case in which (1) all processes are correct, and (2) all processes propose the same value.
\fast unfolds in two ``all-to-leader, leader-to-all'' communication rounds:
\begin{compactenum}
    \item Each process $P_i$ sends a $\langle \textsc{proposal}, v, \mathit{ShareSign}_i(v) \rangle$ message to $P_1$, where $v$ denotes the proposal of $P_i$.
    
    \item If process $P_1$ receives $n$ \textsc{proposal} messages containing the same value $v$, $P_i$ (1) combines the received partial signatures into a threshold signature $\sigma_v$ proving that all $n$ processes have proposed $v$, and (2) broadcasts a $\langle \textsc{fast-decide}, v, \sigma_v \rangle$ to all processes.
    Once a correct process $P_i$ receives a \textsc{fast-decide} message containing $v$, it decides $v$. 
\end{compactenum}
For the sake of completeness, we give the full pseudocode of \fast in \Cref{algorithm:fastest_path}.

\begin{algorithm}
\caption{\fast: Pseudocode for process $P_i$}
\label{algorithm:fastest_path}
\begin{algorithmic} [1]
\State \textbf{Round 1:}

\smallskip
\State \hskip2em \textbf{send} $\langle \textsc{proposal}, \mathit{proposal}_i, \mathit{ShareSign}_i^n(\mathit{proposal}_i) \rangle$ to $P_1$ \label{line:send_proposal_fastest_path}

\medskip
\State \textbf{Round 2:}

\smallskip
\State \hskip2em \textbf{if} $P_i = P_1$: \BlueComment{only $P_1$}
\State \hskip4em \textbf{if} $n$ \textsc{proposal} messages for the same value $v$ are received at the end of Round 1:
\State \hskip6em $\sigma_v \gets \mathit{Combine}^n(\{\mathit{sig} \,|\, \mathit{sig} \text{ is received in a \textsc{proposal} message}\}$
\State \hskip6em \textbf{broadcast} $\langle \textsc{fast-decide}, v, \sigma_v \rangle$

\smallskip
\State \hskip2em \textbf{if} $\langle \textsc{fast-decide}, v, \sigma_v \rangle$ is received from $P_1$ for some value $v$ at the end of Round 2:
\State \hskip4em $\mathit{decision}_i \gets v$ \BlueComment{$P_i$ decides $v$}
\end{algorithmic}
\end{algorithm}

==> sections/overview.tex <==
\section{Overview of \name}

In this section, we give an overview of \name.
First, we introduce \name's building blocks: \emph{phase} and \emph{fallback}.
Second, we describe how \name 

==> sections/strong_intuition.tex <==
\section{\name: Intuition \& Building Blocks}

Roughly speaking, \name consists of three building blocks:
\begin{compactitem}
    \item \fast, \name's fastest path: \fast ensures that, if all processes are correct and they propose the same value, all correct processes decide within $2$ rounds and with only $2n$ exchanged words.
    
    \item \core, the core protocol of \name: \core ensures that, if the actual number of faulty processes is small, all correct processes decide in a small number of rounds, where each round is implemented in the ``all-to-leader, leader-to-all'' communication pattern.
    
    \item \fallback, the fallback protocol of \name: If, during an execution of \core, correct processes determine that there exist $\Omega(n)$ faults, processes start executing \fallback.
    \fallback ensures that all correct processes decide with $O(n^2)$ communication complexity, and $O(f)$ latency complexity.
\end{compactitem}

==> sections/strong_protocol.tex <==
\section{\name = \cert + Adaptive Byzantine Agreement with Weak Validity}

This section presents \name, a strong Byzantine agreement protocol which achieves (1) $O(n \cdot f)$ communication complexity, and (2) $O(f)$ latency complexity.
We build \name as a composition of \cert and an adaptive Byzantine agreement with weak validity.
First, we describe \name, and present its pseudocode.
Then, we prove the correctness and complexity of \name.

\subsection{Protocol Description}

Recall that \cert solves the certification problem with $t_{\mathit{opt}}$ optimistic threshold.

% \begin{algorithm} [ht]
% \caption{Subprotocol $\mathsf{fallback\_certification}$: Pseudocode (for process $P_i$)}
% \label{algorithm:expensive_certification}
% \footnotesize
% \begin{algorithmic} [1]

% \State \textbf{Subprotocol} $\mathsf{fallback\_certification}(\mathsf{Value} \text{ } \mathit{proposal}_i, \mathsf{T\_Signature} \text{ } \mathit{proof}_i)$:
% \State \hskip2em $\mathsf{Boolean}$ $\mathit{started}_i \gets \mathit{false}$

% \medskip
% \State \hskip2em \textbf{Round 1:}
% \State \hskip4em \textbf{if} $\mathit{proof}_i \neq \bot$:
% \State \hskip6em $\mathit{started}_i \gets \mathit{true}$
% \State \hskip6em \textbf{broadcast} $\langle \textsc{proposal}, \mathit{proposal}_i, \mathit{ShareSign}_i^{t + 1}(\mathit{proposal}_i), \mathit{proof}_i \rangle$ \label{line:broadcast_proposal_1}

% \medskip
% \State \hskip2em \textbf{Round 2:}
% \State \hskip4em \textbf{if} $\langle \textsc{proposal}, \cdot, \cdot, \mathsf{T\_Signature} \text{ } \mathit{proof} \rangle$ is received and $\mathit{started}_i = \mathit{false}$:
% \State \hskip6em $\mathit{proof}_i \gets \mathit{proof}$
% \State \hskip6em $\mathit{started}_i \gets \mathit{true}$
% \State \hskip6em \textbf{broadcast} $\langle \textsc{proposal}, \mathit{proposal}_i, \mathit{ShareSign}_i^{t + 1}(\mathit{proposal}_i), \mathit{proof}_i \rangle$ \label{line:broadcast_proposal_2}

% \medskip
% \State \hskip2em \textbf{Round 3:}
% \State \hskip4em \textcolor{blue}{\(\triangleright\) check if the same value is reported by $t + 1$ processes (in both rounds)}
% \State \hskip4em \textbf{if} exists $\mathsf{Value}$ $v$ such that $\langle \textsc{proposal}, v, \mathsf{P\_Signature} \text{ } \mathit{sig}, \cdot \rangle$ is received from $t + 1$ processes: \label{line:common_value_subprotocol}
% \State \hskip6em $\mathsf{T\_Signature}$ $\mathit{fallback\_certificate} \gets \mathit{Combine}^{t + 1}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in a } \textsc{proposal} \text{ message} \} \big)$
% \State \hskip6em \textbf{broadcast} $\langle \textsc{fallback\_certificate}, v, \mathit{fallback\_certificate} \rangle$ \label{line:broadcast_fallback_certificate_subprotocol}
% \State \hskip4em \textbf{else if} $\mathit{started}_i = \mathit{true}$:
% \State \hskip6em \textbf{broadcast} $\langle \textsc{allow-any}, \mathit{ShareSign}_i^{t + 1}(\text{``allow any''}) \rangle$ \label{line:broadcast_allow_any}

% \medskip
% \State \hskip4em \textcolor{blue}{\(\triangleright\) end of the round}
% \State \hskip4em \textbf{if} $\langle \textsc{fallback\_certificate}, \mathsf{Value} \text{ } v', \mathsf{T\_Signature} \text{ } \mathit{fallback\_certificate}' \rangle$ is received:
% \State \hskip6em \textbf{return} $v'$, $\mathit{certificate}'$
% \State \hskip4em \textbf{else if} $\mathit{started}_i = \mathit{true}$:
% \State \hskip6em $\mathsf{T\_Signature}$ $\mathit{certificate}' \gets \mathit{Combine}^{t + 1}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in an } \textsc{allow-any} \text{ message} \} \big)$ \label{line:construct_allow_any_certificate_subprotocol}
% \State \hskip6em \textbf{return} $\mathit{proposal}_i$, $\mathit{certificate}'$

% \State \hskip4em \textbf{else:}
% \State \hskip6em \textbf{return} $\bot$, $\bot$

% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm} [ht]
% \caption{\name: Pseudocode (for process $P_i$)}
% \label{algorithm:strong}
% \footnotesize
% \begin{algorithmic} [1]

% \State \textbf{Variables:}
% \State \hskip2em $\mathsf{Value}$ $\mathit{proposal}_i \gets $ $P_i$'s proposal
% \State \hskip2em $\mathsf{Value}$ $\mathit{proposal\_to\_forward}_i \gets \bot$
% \State \hskip2em $\mathsf{Boolean}$ $\mathit{fast\_certificate\_obtained}_i \gets \mathit{false}$ \BlueComment{states whether a certificate is obtained}
% \State \hskip2em $\mathsf{Certificate}$ $\mathit{certificate}_i \gets \bot$ \BlueComment{obtained certificate}
% \State \hskip2em $\mathsf{T\_Signature}$ $\mathit{culpability\_proof}_i \gets \bot$

% \medskip
% \State \textbf{for} $j = 1$ to $t_{\mathit{opt}} + 1$:
% \State \hskip2em \textbf{invoke} $\text{\cert}_j.\mathsf{start}(\mathit{proposal}_i)$ \BlueComment{in $\text{\cert}_j$, the leader is $P_j$}
% \State \hskip2em \textbf{wait for} $\text{\cert}_j.\mathsf{stop}$

% \State \hskip2em \textbf{if} an $\text{\cert}_j.\mathsf{obtain\_certificate}(\mathsf{Value} \text{ } v', \mathsf{Certificate} \text{ } \Sigma')$ indication is received:
% \State \hskip4em $\mathit{proposal\_to\_forward}_i \gets v'$
% \State \hskip4em $\mathit{certificate}_i \gets \Sigma'$
% \State \hskip4em $\mathit{certificate\_obtained}_i \gets \mathit{true}$

% \medskip
% \State \textbf{Round 1:}
% \State \hskip2em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{false}$:
% \State \hskip4em \textbf{broadcast} $\langle \textsc{help\_req}, \mathit{ShareSign}_i^{t + 1}(\text{``help''}) \rangle$

% \medskip
% \State \textbf{Round 2:}
% \State \hskip2em \textbf{if} received $\langle \textsc{help\_req}, \cdot \rangle$ from $P_j$ and $\mathit{certificate\_obtained} = \mathit{true}$:
% \State \hskip4em \textbf{send} $\langle \textsc{help\_reply}, \mathit{certificate}_i \rangle$ to $P_j$

% \State \hskip2em \textbf{if} received $\langle \textsc{help\_req}, \mathsf{P\_Signature} \text{ } \mathit{sig} \rangle$ from $t + 1$ processes:
% \State \hskip4em $\mathit{culpability\_proof}_i \gets \mathit{Combine}^{t + 1}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in a } \textsc{help\_req} \text{ message} \} \big)$

% \medskip
% \State \textbf{Round 3:}
% \State \hskip2em \textbf{invoke} $\mathsf{fallback\_certification}(\mathit{proposal}_i, \mathit{culpability\_proof}_i)$

% \medskip
% \State \textbf{Round 6:}
% \State \hskip2em Let $\mathsf{Value}$ $\mathit{fallback\_value}$, $\mathsf{Certificate}$ $\mathit{fallback\_certificate}$ be the result of $\mathsf{fallback\_certification}$
% \State \hskip2em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{false}$:
% \State \hskip4em $\mathit{proposal\_to\_forward}_i \gets \mathit{fallback\_value}$
% \State \hskip4em $\mathit{certificate}_i \gets \mathit{fallback\_certificate}$
% \State \hskip2em start the adaptive, closed-box Byzantine agreement with $(\mathit{proposal\_to\_forward}_i, \mathit{certificate}_i)$

% \medskip
% \State \textbf{upon} deciding $\mathsf{Value}$ $v$ from the adaptive, closed-box Byzantine agreement:
% \State \hskip2em $\mathsf{decide}(v)$
% \end{algorithmic}
% \end{algorithm}
\iffalse

\begin{algorithm} [ht]
\caption{\name: Pseudocode (for process $P_i$)}
\label{algorithm:strong_new}
\footnotesize
\begin{algorithmic} [1]

\State \textbf{Variables:}
\State \hskip2em $\mathsf{Value}$ $\mathit{proposal}_i \gets $ $P_i$'s proposal
\State \hskip2em $\mathsf{Value}$ $\mathit{decision}_i \gets \mathit{undecided}$
\State \hskip2em $\mathsf{T\_Signature}$ $\mathit{decision\_proof}_i \gets \bot$
\State \hskip2em $\mathsf{Value}$ $\mathit{commit}_i \gets \bot$
\State \hskip2em $\mathsf{T\_Signature}$ $\mathit{commit\_proof}_i \gets \bot$
\State \hskip2em $\mathsf{Value}$ $\mathit{phase\_decision}_i \gets \bot$

\smallskip
\State \hskip2em $\mathsf{T\_Signature}$ $\mathit{culpability\_proof}_i \gets \bot$
\State \hskip2em $\mathsf{Value}$ $\mathit{fallback\_proposal}_i \gets \bot$
\State \hskip2em $\mathsf{T\_Signature}$ $\mathit{fallback\_proposal\_proof}_i \gets \bot$

% \State \hskip2em $\mathsf{Value}$ $\mathit{proposal\_to\_forward}_i \gets \bot$
% \State \hskip2em $\mathsf{Boolean}$ $\mathit{certificate\_obtained}_i \gets \mathit{false}$ \BlueComment{states whether a certificate is obtained}
% \State \hskip2em $\mathsf{Certificate}$ $\mathit{certificate}_i \gets \bot$ \BlueComment{obtained certificate}
% \State \hskip2em $\mathsf{T\_Signature}$ $\mathit{culpability\_proof}_i \gets \bot$

\medskip
\State \textbf{for} $j = 1$ to $t_{\mathit{opt}} + 1$: \BlueComment{$t_{\mathit{opt}} \leq n - \lceil \frac{n + t + 1}{2} \rceil$}
\State \hskip2em $\mathit{phase\_decision}_i, \mathit{decision\_proof}_i, \mathit{commit}_i, \mathit{commit\_proof}_i \gets \mathsf{phase}(P_j, \mathit{proposal}_i, \mathit{decision}_i, \mathit{commit}_i, \mathit{commit\_proof}_i)$
\State \hskip2em \textbf{if} $\mathit{decision}_i = \mathit{undecided}$ and $\mathit{phase\_decision}_i \neq \mathit{undecided}$:
\State \hskip4em $\mathit{decision}_i \gets \mathit{phase\_decision}_i$

\medskip
\State \textbf{Round 1:}
\State \hskip2em \textbf{if} $\mathit{decision}_i = \mathit{undecided}$: \label{line:check_for_broadcast_help_req}
\State \hskip4em \textbf{broadcast} $\langle \textsc{help\_req}, \mathit{ShareSign}_i^{t + 1}(\text{``help''}) \rangle$ \label{line:broadcast_help_req}

\medskip
\State \textbf{Round 2:}
\State \hskip2em \textbf{if} received $\langle \textsc{help\_req}, \cdot \rangle$ from $P_j$ and $\mathit{decision}_i \neq \mathit{undecided}$:
\State \hskip4em \textbf{send} $\langle \textsc{help\_reply}, \mathit{decision}_i, \mathit{decision\_proof}_i \rangle$ to $P_j$ \label{line:send_help_reply}

\smallskip
\State \hskip2em \textbf{if} received $\langle \textsc{help\_req}, \mathsf{P\_Signature} \text{ } \mathit{sig} \rangle$ from $t + 1$ processes:
\State \hskip4em $\mathit{culpability\_proof}_i \gets \mathit{Combine}^{t + 1}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in a } \textsc{help\_req} \text{ message} \} \big)$ \label{line:culpability_proof}
\State \hskip4em \textbf{broadcast} $\langle \textsc{fallback}, \mathit{culpability\_proof}_i, \mathit{decision}_i, \mathit{decision\_proof}_i \rangle$
\State \hskip4em $\mathit{fallback\_start}_i \gets \mathsf{time\_now} + 2\delta$

\medskip
\State \textbf{Round 3:}
\State \hskip2em \textbf{if} received $\langle \textsc{help\_reply}, \mathsf{Value} \text{ } v, \mathsf{T\_Signature} \text{ } \mathit{QC}_{\mathit{finalized}}(v) \rangle$ and $\mathit{decision}_i = \mathit{undecided}$: \label{line:receive_help_reply}
\State \hskip4em $\mathit{decision}_i \gets v$
\State \hskip4em $\mathit{decision\_proof}_i \gets \mathit{QC}_{\mathit{finalized}}(v)$

\smallskip
\State \hskip2em $\mathit{fallback\_proposal}_i \gets \mathit{decided}_i$
\State \hskip2em \textbf{while} $\mathit{fallback\_start} > \mathsf{time\_now}$:
\State \hskip4em \textbf{if} received $\langle \textsc{fallback}, \mathsf{T\_Signature} \text{ } \mathit{culpability\_proof}, \mathsf{Value} \text{ } v, \mathsf{T\_Signature} \text{ } \mathit{QC}_{\mathit{finalized}}(v) \rangle$:
\State \hskip6em \textbf{if} $\mathit{decision}_i = \mathit{undecided}$ and $\mathit{QC}_{\mathit{finalized}}(v) \neq \bot$:
\State \hskip8em $\mathit{fallback\_proposal}_i \gets v$
\State \hskip8em $\mathit{fallback\_proposal\_proof}_i \gets \mathit{QC}_{\mathit{finalized}}(v)$

\State \hskip6em \textbf{if} $\mathit{fallback\_start}_i = \infty$:
\State \hskip8em \textbf{broadcast} $\langle \textsc{fallback}, \mathit{culpability\_proof}, \mathit{decision}_i, \mathit{decision\_proof}_i \rangle$
\State \hskip8em $\mathit{fallback\_start}_i \gets \mathsf{time\_now} + 2\delta$

\smallskip
\State \hskip2em $\mathsf{Value}$ $\mathit{fallback\_decision} \gets $ $\mathcal{A}_{\mathit{fallback}}$ with $\delta' = 2\delta$ and initial value $\mathit{fallback\_proposal}_i$
\State \hskip2em \textbf{if} $\mathit{fallback\_decision}$ is valid and $\mathit{decision}_i = \mathit{undecided}$:
\State \hskip4em $\mathit{decision}_i \gets \mathit{fallback\_decision}$
\State \hskip2em \textbf{else if} $\mathit{decision}_i = \mathit{undecided}$:
\State \hskip4em $\mathit{decision}_i \gets \bot$
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%
% end Strong algorithm
%%%%%%%%%%%%%%

%%%%%%%%%%%%%
% Phase algorithm
%%%%%%%%%%%%%
\begin{algorithm} [ht]
\caption{$\mathsf{phase}$: Pseudocode (for process $P_i$)}
\label{algorithm:phase}
\footnotesize
\begin{algorithmic} [1]

\State \textbf{Parameters:}
\State \hskip2em $\mathsf{Process}$ $\mathit{leader}_i$
\State \hskip2em $\mathsf{Value}$ $\mathit{proposal}_i$
\State \hskip2em $\mathsf{Value}$ $\mathit{decision}_i$
\State \hskip2em $\mathsf{T\_Signature}$ $\mathit{decision\_proof}_i$
\State \hskip2em $\mathsf{Value}$ $\mathit{commit}_i$
\State \hskip2em $\mathsf{T\_Signature}$ $\mathit{commit\_proof}_i$

\medskip
\State \textbf{Variables:}
\State \hskip2em $\mathit{certificate\_proposal}_i \gets \bot$
\State \hskip2em $\mathit{certificate}_i \gets \bot$
% \State \hskip2em $\mathsf{Value}$ $\mathit{proposal}_i \gets $ $P_i$'s proposal
% \State \hskip2em $\mathsf{Value}$ $\mathit{proposal\_to\_forward}_i \gets \bot$
% \State \hskip2em $\mathsf{Boolean}$ $\mathit{certificate\_obtained}_i \gets \mathit{false}$ \BlueComment{states whether a certificate is obtained}
% \State \hskip2em $\mathsf{Certificate}$ $\mathit{certificate}_i \gets \bot$ \BlueComment{obtained certificate}
% \State \hskip2em $\mathsf{T\_Signature}$ $\mathit{culpability\_proof}_i \gets \bot$

\medskip
\State \textbf{invoke} $\text{\cert}.\mathsf{start}(\mathit{proposal}_i)$, where the leader is $\mathit{leader}_i$ and the optimistic threshold is $t_{\mathit{opt}}$
\State \textbf{wait for} $\text{\cert}.\mathsf{stop}$
\State \textbf{if} $P_i = \mathit{leader}_i$ and a $\text{\cert}.\mathsf{obtain\_certificate}(\mathsf{Value} \text{ } v, \mathsf{Certificate} \text{ } \mathit{certificate})$ indication is received:
\State \hskip2em $\mathit{certificate\_proposal}_i \gets \mathit{v}$
\State \hskip2em $\mathit{certificate}_i \gets \mathit{certificate}$

\medskip
\State \textbf{Round 1:}
\State \hskip2em \textbf{if} $P_i = \mathit{leader}_i$ and $\mathit{certificate}_i \neq \bot$ and $\mathit{decision}_i = \bot$:
\State \hskip4em \textbf{broadcast} $\langle \textsc{proposal}, \mathit{certificate\_proposal}_i, \mathit{certificate}_i \rangle$

\medskip
\State \textbf{Round 2:}
\State \hskip2em \textbf{if} received $\langle \textsc{proposal}, \mathsf{Value} \text{ } v, \mathsf{Certificate} \text{ } \mathit{certificate} \rangle$ from $\mathit{leader}_i$ such that $\mathsf{verify}(v, \mathit{certificate}) = \mathit{true}$:
\State \hskip4em \textbf{if} $\mathit{commit}_i = \bot$:
\State \hskip6em \textbf{send} $\langle \textsc{vote}, v, \mathit{ShareSign}_i^{\lceil \frac{n + t + 1}{2} \rceil}(v) \rangle$ to $\mathit{leader}_i$
\State \hskip4em \textbf{else:}
\State \hskip6em \textbf{send} $\langle \textsc{commit}, \mathit{commit}_i, \mathit{commit\_proof}_i \rangle$ to $\mathit{leader}_i$

\medskip
\State \textbf{Round 3:}
\State \hskip2em \textbf{if} $P_i = \mathit{leader}_i$:
\State \hskip4em \textbf{if} received $\langle \textsc{commit}, \mathsf{Value} \text{ } v, \mathsf{T\_Signature} \text{ } \mathit{QC}_{\mathit{commit}}(v) \rangle$:
\State \hskip6em \textbf{broadcast} $\langle \textsc{commit}, v, \mathit{QC}_{\mathit{commit}}(v) \rangle$
\State \hskip4em \textbf{else if} exists $\mathsf{Value}$ $v$ such that $\lceil \frac{n + t + 1}{2} \rceil$ $\langle \textsc{proposal}, v, \cdot \rangle$ messages are received:
\State \hskip6em $\mathsf{T\_Signature}$ $\mathit{QC}_{\mathit{commit}}(v) \gets \mathit{Combine}^{\lceil \frac{n + t + 1}{2} \rceil}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in the \textsc{proposal} messages}   \} \big)$
\State \hskip6em \textbf{broadcast} $\langle \textsc{commit}, v, \mathit{QC}_{\mathit{commit}}(v) \rangle$

\medskip
\State \textbf{Round 4:}
\State \hskip2em \textbf{if} received $\langle \textsc{commit}, \mathsf{Value} \text{ } v, \mathsf{T\_Signature} \text{ } \mathit{QC}_{\mathit{commit}}(v) \rangle$:
\State \hskip4em \textbf{send} $\langle \textsc{decide}, v, \mathit{ShareSign}_i^{\lceil \frac{n + t + 1}{2} \rceil}(v) \rangle$ to $\mathit{leader}_i$
\State \hskip4em \textbf{if} $\mathit{commit}_i = \bot$:
\State \hskip6em $\mathit{commit}_i \gets v$
\State \hskip6em $\mathit{commit\_proof}_i \gets \mathit{QC}_{\mathit{commit}}(v)$

\medskip
\State \textbf{Round 5:}
\State \hskip2em \textbf{if} $P_i = \mathit{leader}_i$:
\State \hskip4em \textbf{if} exists $\mathsf{Value}$ $v$ such that $\lceil \frac{n + t + 1}{2} \rceil$ $\langle \textsc{decide}, v, \cdot \rangle$ messages are received:
\State \hskip6em $\mathsf{T\_Signature}$ $\mathit{QC}_{\mathit{finalized}}(v) \gets \mathit{Combine}^{\lceil \frac{n + t + 1}{2} \rceil}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in the \textsc{decide} messages}   \} \big)$
\State \hskip6em \textbf{broadcast} $\langle \textsc{finalized}, v, \mathit{QC}_{\mathit{commit}}(v) \rangle$

\smallskip
\State \hskip2em \textcolor{blue}{\(\triangleright\) end of the round}
\State \hskip2em \textbf{if} received $\langle \textsc{finalized}, \mathsf{Value} \text{ } v, \mathsf{T\_Signature} \text{ } \mathit{QC}_{\mathit{finalized}}(v) \rangle$ from $\mathit{leader}_i$:
\State \hskip4em $\mathit{decision}_i \gets v$
\State \hskip4em $\mathit{decision\_proof}_i \gets \mathit{QC}_{\mathit{finalized}}(v)$

\smallskip
\State \hskip2em \textbf{return} $(\mathit{decision}_i, \mathit{decision\_proof}_i, \mathit{commit}_i, \mathit{commit\_proof}_i)$ 
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%
% end Phase algorithm
%%%%%%%%%%%
\fi

%%%%%%%%%%%
% new Strong protocol
%%%%%%%%%%%
\begin{algorithm} [ht]
\caption{\name: Pseudocode (for process $P_i$)}
\label{algorithm:strong_new}
\footnotesize
\begin{algorithmic} [1]

\State \textbf{Variables:}
\State \hskip2em $\mathsf{Value}$ $\mathit{proposal}_i \gets $ $P_i$'s proposal
\State \hskip2em $\mathsf{Value}$ $\mathit{proposal\_to\_forward}_i \gets \bot$
\State \hskip2em $\mathsf{Boolean}$ $\mathit{certificate\_obtained}_i \gets \mathit{false}$ \BlueComment{states whether a certificate is obtained}
\State \hskip2em $\mathsf{Certificate}$ $\mathit{certificate}_i \gets \bot$ \BlueComment{obtained certificate}
%\State \hskip2em $\mathsf{T\_Signature}$ $\mathit{culpability\_proof}_i \gets \bot$

\medskip
\State \textbf{for} $j = 1$ to $t_{\mathit{opt}} + 1$:
\State \hskip2em \textbf{invoke} $\text{\cert}_j.\mathsf{start}(\mathit{proposal}_i)$ \BlueComment{in $\text{\cert}_j$, the leader is $P_j$}
\State \hskip2em \textbf{wait for} $\text{\cert}_j.\mathsf{stop}$

\State \hskip2em \textbf{if} a $\text{\cert}_j.\mathsf{obtain\_certificate}(\mathsf{Value} \text{ } v', \mathsf{Certificate} \text{ } \Sigma')$ indication is received:
\State \hskip4em $\mathit{proposal\_to\_forward}_i \gets v'$; $\mathit{certificate}_i \gets \Sigma'$; $\mathit{certificate\_obtained}_i \gets \mathit{true}$ \label{line:fast_certificate_obtained}


\medskip
\State \textbf{Round 1:}
\State \hskip2em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{false}$: \label{line_new:check_for_broadcast_help_req}
\State \hskip4em \textbf{broadcast} $\langle \textsc{help\_req} \rangle$ \label{line_new:broadcast_help_req}

\medskip
\State \textbf{Round 2:}
\State \hskip2em \textbf{if} received $\langle \textsc{help\_req} \rangle$ from $P_j$:
\State \hskip4em \textbf{send} $\langle \textsc{help\_reply}, \mathit{proposal\_to\_forward}_i, \mathit{certificate}_i, \mathit{ShareSign}_i^{t + 1}(\mathit{proposal}_i) \rangle$ to $P_j$ \label{line:send_help_reply}

\medskip
\State \textbf{Round 3:}
\State \hskip2em \textbf{if} received $\langle \textsc{help\_reply}, \mathsf{Value} \text{ } v, \mathsf{Certificate} \text{ } \mathit{certificate}, \cdot \rangle$ such that $\mathit{certificate} \neq \bot$:
\State \hskip4em $\mathit{proposal\_to\_forward}_i \gets v$; $\mathit{certificate}_i \gets \mathit{certificate}$; $\mathit{certificate\_obtained}_i \gets \mathit{true}$

\smallskip
\State \hskip2em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{false}$ and exists $\mathsf{Value}$ $v$ with $t + 1$ $\langle \textsc{help\_reply}, v, \cdot, \cdot \rangle$ messages received:  \label{line:check_for_broadcast_final_certificate} 
\State \hskip4em $\mathit{certificate\_obtained}_i \gets \mathit{true}$
\State \hskip4em $\mathit{proposal\_to\_forward}_i \gets v$
\State \hskip4em $\mathit{certificate}_i \gets \mathit{Combine}^{t + 1}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in the aforementioned $t + 1$ \textsc{help\_reply} messages}   \} \big)$ \label{line:obtain_specific_certificate}
\State \hskip4em \textbf{broadcast} $\langle \textsc{final\_certificate}, \mathit{proposal\_to\_forward}_i, \mathit{certificate}_i \rangle$

\smallskip
\State \hskip2em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{false}$: \label{line:check_for_broadcast_allow_any}
\State \hskip4em \textbf{broadcast} $\langle \textsc{allow-any}, \mathit{ShareSign}_i^{t + 1}(\text{``allow any''}) \rangle$ \label{line:broadcast_allow_any}

\medskip
\State \textbf{Round 4:}
\State \hskip2em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{false}$:
\State \hskip4em \textbf{if} received $\langle \textsc{final\_certificate}, \mathsf{Value} \text{ } v, \mathsf{Certificate} \text{ } \mathit{certificate}_i \rangle$:
\State \hskip6em $\mathit{proposal\_to\_forward}_i \gets v$; $\mathit{certificate}_i \gets \mathit{certificate}$; $\mathit{certificate\_obtained}_i \gets \mathit{true}$
\State \hskip4em \textbf{else:}
\State \hskip6em $\mathit{proposal\_to\_forward}_i \gets \mathit{proposal}_i$
\State \hskip6em $\mathit{certificate}_i \gets \mathit{Combine}^{t + 1}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in an \textsc{allow-any} message}   \} \big)$ \label{line:obtain_general_certificate}
\State \hskip2em start the adaptive, closed-box Byzantine agreement with $\mathit{proposal\_to\_forward}_i$, $\mathit{certificate}_i$ \label{line:propose_to_adaptive}

% \State \hskip4em start the adaptive, closed-box Byzantine agreement with $\mathit{proposal\_to\_forward}_i$, $\mathit{certificate}_i$

% \State \hskip2em \textbf{else if} received $\langle \textsc{final\_certificate}, \mathsf{Value} \text{ } v, \mathsf{Certificate} \text{ } \mathit{certificate} \rangle$:
% \State \hskip4em start the adaptive, closed-box Byzantine agreement with $v$, $\mathit{certificate}$
% \State \hskip2em \textbf{else:}
% \State \hskip4em $\mathit{certificate}_i \gets \mathit{Combine}^{t + 1}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in an \textsc{allow-any} message}   \} \big)$ \label{line:slow_negative_certificate}
% \State \hskip4em start the adaptive, closed-box Byzantine agreement with $\mathit{proposal}_i$, $\mathit{certificate}_i$


% \State \hskip2em \textbf{if} received $\langle \textsc{help\_req}, \cdot \rangle$ from $P_j$ and $\mathit{certificate\_obtained}_i = \mathit{true}$:
% \State \hskip4em \textbf{send} $\langle \textsc{help\_reply}, \mathit{proposal\_to\_forward}_i, \mathit{certificate}_i \rangle$ to $P_j$

% \State \hskip2em \textbf{if} received $\langle \textsc{help\_req}, \mathsf{P\_Signature} \text{ } \mathit{sig} \rangle$ from $t + 1$ processes:
% \State \hskip4em $\mathit{culpability\_proof}_i \gets \mathit{Combine}^{t + 1}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in a } \textsc{help\_req} \text{ message} \} \big)$

% \medskip
% \State \textbf{Round 3:}
% \State \hskip2em \textbf{if} received $\langle \textsc{help\_reply}, \mathsf{Value} \text{ } v, \mathsf{Certificate} \text{ } \mathit{certificate} \rangle$ and $\mathit{certificate\_obtained}_i = \mathit{false}$:
% \State \hskip4em $\mathit{proposal\_to\_forward}_i \gets v$; $\mathit{certificate}_i \gets \mathit{certificate}$; $\mathit{certificate\_obtained}_i \gets \mathit{true}$

% \smallskip
% \State \hskip2em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{false}$: \label{line:check_for_broadcast_another}
% \State \hskip4em \textbf{broadcast} $\langle \textsc{another\_help\_req}, \mathit{proposal}_i, \mathit{ShareSign}_i^{t + 1}(\mathit{proposal}_i), \mathit{culpability\_proof}_i \rangle$ \label{line:broadcast_another}

% \medskip
% \State \textbf{Round 4:}
% \State \hskip2em \textbf{if} received $\langle \textsc{another\_help\_req}, \cdot, \cdot, \mathsf{T\_Signature} \text{ } \mathit{culpability\_proof} \rangle$:
% \State \hskip4em $\mathit{culpability\_proof}_i \gets \mathit{culpability\_proof}$
% \State \hskip4em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{true}$: \label{line:check_for_another_help_reply}
% \State \hskip6em \textbf{broadcast} $\langle \textsc{another\_help\_reply}, \mathit{proposal\_to\_forward}_i, \mathit{certificate}_i \rangle$ \label{line:broadcast_another_help_reply}

% \medskip
% \State \textbf{Round 5:}
% \State \hskip2em \textbf{if} received $\langle \textsc{another\_help\_reply}, \mathsf{Value} \text{ } v, \mathsf{Certificate} \text{ } \mathit{certificate} \rangle$ and $\mathit{certitificate\_obtained}_i = \mathit{false}$: \label{line:receive_another_help_reply}
% \State \hskip4em $\mathit{proposal\_to\_forward}_i \gets v$; $\mathit{certificate}_i \gets \mathit{certificate}$; $\mathit{certificate\_obtained}_i \gets \mathit{true}$ \label{line:obtain_certificate_another_help_reply}

% \smallskip
% \State \hskip2em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{false}$ and exists $\mathsf{Value}$ $v$ with $t + 1$ $\langle \textsc{another\_help\_req}, v, \cdot, \cdot \rangle$ messages received: \label{line:receive_t+1}
% \State \hskip4em $\mathit{certificate\_obtained}_i \gets \mathit{true}$ \label{line:obtain_certificate_t+1}
% \State \hskip4em $\mathit{proposal\_to\_forward}_i \gets v$
% \State \hskip4em $\mathit{certificate}_i \gets \mathit{Combine}^{t + 1}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in the aforementioned $t + 1$ \textsc{another\_help\_req} messages}   \} \big)$ \label{line:slow_positive_certificate}


% \smallskip
% \State \hskip2em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{true}$ and $\mathit{culpability\_proof}_i \neq \bot$:
% \State \hskip4em \textbf{broadcast} $\langle \textsc{final\_certificate}, \mathit{proposal\_to\_forward}_i, \mathit{certificate}_i \rangle$
% % \State \hskip4em start the adaptive, closed-box ($2\delta$) Byzantine agreement with $\mathit{proposal\_to\_forward}_i$, $\mathit{certificate}_i$
% \State \hskip2em \textbf{else if} $\mathit{certificate\_obtained}_i = \mathit{false}$: \label{line:check_for_broadcast_allow_any}
% \State \hskip4em \textbf{broadcast} $\langle \textsc{allow-any}, \mathit{ShareSign}_i^{t + 1}(\text{``allow any''}) \rangle$ \label{line:broadcast_allow_any}

% \medskip
% \State \textbf{Round 6:}
% % \State \hskip2em \textbf{if} the adaptive, closed-box Byzantine agreement is not previously started:
% \State \hskip2em \textbf{if} $\mathit{certificate\_obtained}_i = \mathit{true}$:
% \State \hskip4em start the adaptive, closed-box Byzantine agreement with $\mathit{proposal\_to\_forward}_i$, $\mathit{certificate}_i$

% \State \hskip2em \textbf{else if} received $\langle \textsc{final\_certificate}, \mathsf{Value} \text{ } v, \mathsf{Certificate} \text{ } \mathit{certificate} \rangle$:
% \State \hskip4em start the adaptive, closed-box Byzantine agreement with $v$, $\mathit{certificate}$
% \State \hskip2em \textbf{else:}
% \State \hskip4em $\mathit{certificate}_i \gets \mathit{Combine}^{t + 1}\big( \{ \mathit{sig} \,|\, \mathit{sig} \text{ is received in an \textsc{allow-any} message}   \} \big)$ \label{line:slow_negative_certificate}
% \State \hskip4em start the adaptive, closed-box Byzantine agreement with $\mathit{proposal}_i$, $\mathit{certificate}_i$

\medskip
\State \textbf{upon} deciding $\mathsf{Value}$ $v$ from the adaptive, closed-box Byzantine agreement:
\State \hskip2em $\mathsf{decide}(v)$ \label{line:decide_strong}
\end{algorithmic}
\end{algorithm}
